Population synthesis of Galactic pulsars with machine learning

This thesis work represents the first efforts to combine population synthesis studies of the Galactic isolated neutron stars with deep-learning techniques with the aim of better understanding neutron-star birth properties and evolution. In particular, we develop a flexible population-synthesis framework to model the dynamical and magneto-rotational evolution of neutron stars, their emission in radio and their detection with radio telescopes. We first study the feasibility of using deep neural networks to infer the dynamical properties at birth and then explore a simulation-based inference approach to predict the birth magnetic-field and spin-period distributions and the late-time magnetic-field decay for the observed radio pulsar population. Our results for the birth magneto-rotational properties agree with the findings of previous works while we constrain the late-time evolution of the magnetic field in neutron stars for the first time. Moreover, this thesis also studies possible scenarios to explain the puzzling nature of recently discovered periodic radio sources with very long periods of the order of thousands of seconds. In particular, by assuming a neutron-star origin, we study the spin-period evolution of a newborn neutron star interacting with a supernova fallback disk and find that the combination of strong, magnetar-like magnetic fields and moderate accretion rates can lead to very large spin periods on timescales of ten thousands of years. Moreover, we perform population synthesis studies to assess the possibility for these sources to be either neutron stars or magnetic white dwarfs emitting coherently through magnetic dipolar losses. These discoveries have opened up a new perspective on the neutron-star population and have started to question our current understanding of how coherent radio emission is produced in pulsar magnetospheres.

==> Chapters/Chapter_NS_theory.tex <==
\chapter{Neutron stars, radio emission and detection} % Main chapter title

\label{Chapter2} % For referencing the chapter elsewhere, use \ref{Chapter2} 

%----------------------------------------------------------------------------------------

In this chapter we will explore the basics of neutron star physics and our current understanding of how they evolve, emit electromagnetic radiation, with particular focus on the radio emission, and how we can detect them. These are the main ingredients necessary to develop a population synthesis model that describe the observed Galactic neutron star population.  

\section{The magnetosphere} \label{sec:ch2_magnetosphere}

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{magnetosphere_cerutti.pdf}
\caption[Sketch of the ideal force-free magnetosphere]{Sketch of the ideal force-free magnetosphere of the aligned pulsar. The main elements are: (i) The closed field line region (grey, and black field lines) lying between the star surface and the light cylinder. This zone is dead and does not participate to the pulsar activity. (ii) The open field line region (red and blue field lines) extending beyond the light cylinder. As particles are accelerated along the open field line region they emit electromagnetic radiation. (iii) The equatorial current sheet (green) between the opposite magnetic fluxes in the open field line region. It splits at the light cylinder into two separatrix current sheets that go around the closed zone, between the last open and the first closed field lines \citep[see][for further details]{Cerutti2017} \citep[Figure adapted from][]{Cerutti2017}.}
\label{fig:ch2_sketch_magnetosphere}
\end{figure*}
%----------------------------------------------------

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{3D_magnetosphere.pdf}
\caption[Simulated 3D force-free magnetosphere]{Slices through the simulated force-free magnetosphere of a neutron star with inclination angle of $60^{\circ}$ between the magnetic dipole moment and the rotation axis. The ﬁeld lines in the horizontal and vertical slices are shown; color represents the magnetic ﬁeld component perpendicular to the slices. A sample three-dimensional magnetic ﬂux tube is traced in white \citep[Figure taken from][]{Spitkovsky2006}.}
\label{fig:ch2_3D_magnetosphere}
\end{figure*}
%----------------------------------------------------

The magnetosphere of a neutron star is a complex and dynamic region filled with magnetized plasma where strong magnetic fields interact with the surrounding environment. It envelopes the entire star extending from the stellar surface up to several thousands of kilometers. Unlike Earth's magnetosphere, which is primarily influenced by the interaction with the solar wind, neutron star magnetospheres can encounter various external influences, including the interstellar medium, accretion disks, and even companion stars in binary systems.
\cite{Deutsch1955} was the first to study analytically the structure of the electromagnetic field surrounding an isolated rotating magnetized star with a misaligned magnetic dipole moment in a vacuum. Later, \cite{Goldreich1969} described the pulsar electrodynamics in the simplest case of a rotating magnetic dipole, aligned with the rotational axis, surrounded by a charge-separated plasma.
In general analytical solutions for the magnetospheric structure are possible only in very simplified and ideal cases. To fully study the overall geometry of the electromagnetic fields and how the surrounding plasma interacts with and influences them, numerical simulations are required. \cite{Contopoulos1999} were the first to present a numerical, realistic configuration for an aligned rotator in the force-free approximation (see below). His work was the first step towards more realistic 3D simulations that were able to quantitatively consider the effects of the misalignment between rotation and magnetic axes \citep[see Figure~\ref{fig:ch2_3D_magnetosphere} and][]{Spitkovsky2006, Philippov2014}. 
Understanding the structure and dynamics of neutron star magnetospheres is crucial for comprehending a wide range of phenomena associated with these celestial objects. In particular, the intricate interplay between the magnetic field and the highly energetic particles in the surrounding plasma leads to the generation of electromagnetic radiation across different wavelengths from radio to gamma rays. For more detailed reviews about pulsar magnetosphere see for example \cite{Petri2016, Petri2020}.
 
To gain an insight into the magnetosphere's structure we consider a neutron star initially surrounded by vacuum spinning with angular frequency $\omega = 2 \pi / P$. The neutron star is endowed with a strong magnetic field. However to define this magnetic field we need to make a distinction between two reference frames: an inertial reference frame of an external observer and a reference frame co-rotating with the star. For simplicity we consider the latter to be sufficiently small compared to the star's size and not so far from the axis of rotation as to be considered locally inertial. The position of the co-rotating frame can be described by a distance vector, $\boldsymbol{r}$, originating $\boldsymbol{r}$ at the centre of the neutron star. With these considerations, the electromagnetic fields as measured by the two observers can be linked by the Lorentz transformations \citep{Jackson1998}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_B}
    \boldsymbol{B} = \gamma_{\rm rot} \left(\boldsymbol{B}' + \boldsymbol{\beta}_{\rm rot} \times \boldsymbol{E}' \right) - \frac{\gamma_{\rm rot}^2}{\gamma_{\rm rot} + 1} \boldsymbol{\beta}_{\rm rot} (\boldsymbol{\beta}_{\rm rot} \cdot \boldsymbol{B}'),
\end{align}
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_E}
    \boldsymbol{E} = \gamma_{\rm rot} \left(\boldsymbol{E}' - \boldsymbol{\beta}_{\rm rot} \times \boldsymbol{B}' \right) - \frac{\gamma_{\rm rot}^2}{\gamma_{\rm rot} + 1} \boldsymbol{\beta}_{\rm rot} (\boldsymbol{\beta}_{\rm rot} \cdot \boldsymbol{E}'),
\end{align}
%--------------------------------------------------------------
where $\boldsymbol{E}$ and $\boldsymbol{B}$ are the fields measured by an external observer, while $\boldsymbol{E}'$ and $\boldsymbol{B}'$ are the fields measured in the co-rotating frame, $\boldsymbol{\beta}_{\rm rot} = (\boldsymbol{\omega} \times \boldsymbol{r}) / c$ is the ratio of the rotational velocity to the speed of light $c$ and $\gamma_{\rm rot} = 1 / (1 - \beta_{\rm rot}^2)^{1/2}$ is the corresponding Lorentz factor. 
If we consider the neutron star interior or we stay in the proximity of its surface, for typical observed spin periods we have that $\beta_{\rm rot} \equiv |\boldsymbol{\beta}_{\rm rot}| \ll 1$. Therefore the transformations above assume the simplified form:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_B_1}
    \boldsymbol{B} \sim \left(\boldsymbol{B}' + \boldsymbol{\beta}_{\rm rot} \times \boldsymbol{E}' \right),
\end{align}
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_E_1}
    \boldsymbol{E} \sim \left(\boldsymbol{E}' - \boldsymbol{\beta}_{\rm rot} \times \boldsymbol{B}' \right),
\end{align}
%--------------------------------------------------------------
where we neglected second order terms in $\beta_{\rm rot}$ and considered $\gamma_{\rm rot} \sim 1$.

Little is known about the magnetic field geometry inside the neutron star. In the exterior, the magnetic field is typically described by a combination of multipolar components. As the higher-order multipoles decay faster with distance from the stellar surface, the dipolar component probably dominates the magnetic field geometry at a large scale. For the sake of simplicity we consider that in the neutron star's co-rotating frame the magnetic field is purely dipolar.
In this case the formula that relates the magnetic moment $\boldsymbol{\mu}$ with the strength of the magnetic field $\boldsymbol{B}'$ is given by:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_B_dipole}
\boldsymbol{B}'(\boldsymbol{r}) = \frac{3 (\boldsymbol{r} \cdot \boldsymbol{\mu} ) \boldsymbol{r}}{r^5} - \frac{ \boldsymbol{\mu} }{r^3}. 
\end{align}  
%-----------------------------------------------------------------
We further simplify by assuming a configuration with the magnetic moment $\boldsymbol{\mu}$ aligned with the rotation axis of the star. We will call this an aligned rotator.
In spherical coordinates $(r, \theta, \phi)$ with $\theta$ being the angle computed from the magnetic moment axis (or spin axis in the aligned case) and $\phi$ the azimuthal angle, the dipolar magnetic field can be expressed as:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_B_dipole_sph_coord}
    \boldsymbol{B}'(r, \theta) = \frac{\mu}{r^3} \begin{bmatrix}
           2 \cos{\theta} \\
           \sin{\theta} \\
           0
         \end{bmatrix}.
\end{align}
%--------------------------------------------------------------

Due to the abundance of free charges in its interior, as a first approximation a neutron star can be considered as a perfect conductor. Therefore in the co-rotating frame, the internal electric field has to vanish so that in the neutron star interior the following equations are valid:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_B_2}
    \boldsymbol{B} \sim \boldsymbol{B}',
\end{align}
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_lorentz_transf_E_2}
    \boldsymbol{E} \sim - \boldsymbol{\beta}_{\rm rot} \times \boldsymbol{B}' = - \frac{\boldsymbol{\omega} \times \boldsymbol{r}}{c} \times \boldsymbol{B}'.
\end{align}
%--------------------------------------------------------------
In other words, a perfect conductor rotating in a magnetic field behaves as a unipolar inductor converting the rotational energy into electrical energy. As seen by an inertial external observer the rotation of the star induces an electric field inside the star and the free charges inside rearrange themselves under its action. In particular, on the surface of the star particles of opposite charges are driven to the polar and equatorial regions respectively according to their signs. This creates a quadrupolar electric potential, $V$, on the surface that can be derived from $\boldsymbol{E} = - \boldsymbol{\nabla} V$. 

In particular, for an aligned rotator, from Equation~\eqref{eq:ch2_lorentz_transf_E_2}, the $\theta$ component of the electric field computed at the surface is given by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_E_theta_surf}
E_{\theta} = - \frac{\omega R_{\rm NS} \sin{\theta} B_r}{c}.
\end{align}
%--------------------------------------------------------------
This determines the electrostatic potential drop with latitude on the stellar surface that can be computed considering that $E_{\theta} = 1/r (\partial V / \partial \theta) $ and integrating over the coordinate $\theta$. 
By using the radial component of the surface dipole magnetic field in Equation~\eqref{eq:ch2_B_dipole_sph_coord}, $B_r = 2 \mu \cos{\theta} / R_{\rm NS}^3$, we find \citep{Backus1956, Goldreich1969, Cerutti2017}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_unipolar_potential}
    V(R_{\rm NS}, \theta) - V(R_{\rm NS}, 0) = \int_0^\theta E_{\theta} R_{\rm NS} {\rm d}\theta = \frac{\omega \mu}{2 R_{\rm NS} c} \sin^2{\theta},
\end{align}
%--------------------------------------------------------------
where $V(R_{\rm NS}, 0) \equiv V_{\rm p}$ is the value of the electric potential at the pole.
This charge redistribution induces an external quadrupolar electric field with a strong component parallel to the magnetic field lines. As shown by \cite{Goldreich1969} this component of the electric field is strong enough to overcome gravity and pull out charged particles from the neutron star surface unless strong cohesive forces prevent them from escaping. This happens primarily for the electrons and protons as, in the presence of a strong magnetic field, heavier ions in the surface layer can rearrange themselves to form a dense and strongly bound molecular lattice \citep[see][and reference therein]{Ruderman1975}. Even if considered as a simplified and ideal case, the result from \cite{Goldreich1969} implies that a vacuum region around a neutron star cannot be maintained and a magnetosphere filled with conducting plasma has to surround the star.

As charges are extracted from the surface they are accelerated up to relativistic speeds along the magnetic field lines by the induced electric field. By moving along curved field lines these charges produce gamma-ray photons by curvature radiation \citep{Ruderman1975} or the inverse-Compton process by up-scattering lower energy photons \citep{Daugherty1986}. In the presence of strong magnetic fields gamma-ray photons can transform into electron-positron pairs, if the photon energy exceeds the threshold $E_{\gamma} \geq 2 m_e c^2$ where $m_e$ is the electron mass. This generation of new particles then produces new photons and pairs leading to a pair cascade that populates the magnetosphere with co-rotating highly conducting plasma. Assuming a continuous supply of charges, as the magnetosphere is replenished with perfectly conducting plasma (predominantly formed by $e^{-} \, e^{+}$ pairs) the electric field component along the magnetic field lines gets screened so that in a steady state one expects the condition $\boldsymbol{E} \cdot \boldsymbol{B} = 0$ to be satisfied. This prevents any further acceleration of particles along the field lines so that these can be considered equipotential lines. In this ideal case, called force-free limit, the magnetosphere is sufficiently populated with plasma for the conductivity in the medium to become infinite. Moreover, the electromagnetic field dominates the dynamics of the magnetosphere by several orders of magnitude with respect to pressure, gravity and inertia.
The unipolar induction mechanism on the other hand induces an electric field perpendicular to the magnetic field lines that lead to charge separation also in the magnetosphere. 

However, the flow of plasma in the magnetosphere has a retroactive effect on the electromagnetic field structure around the neutron star.  
As we move further away from the neutron star surface, the approximations and the electromagnetic field configuration outlined above break down. As the rotational velocity approaches the speed of light plasma co-rotation becomes impossible and a co-rotating frame cannot be defined anymore. We define an imaginary cylindrical surface called light cylinder, with the axis parallel to the rotation axis of the star. The radius of the light cylinder corresponds to the distance where the co-rotating speed is equal to the speed of light:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_light_cylinder}
    r_{\rm lc} = \frac{c}{\omega} \simeq \unit[4.77 \times 10^9]{cm} \left( \frac{P}{\unit[1]{s}} \right).
\end{align}
%--------------------------------------------------------------

Near the light cylinder plasma inertia due to the approaching of the speed of light becomes relevant and the plasma is not able to stay in co-rotation. In particular, the plasma drags the magnetic field causing the field lines to sweep back in the azimuthal direction and spiral around the star (see Figure~\ref{fig:ch2_3D_magnetosphere}). This produces a toroidal magnetic field component. Furthermore, the co-rotating charges and these inertial effects create currents which modify the magnetic field configuration. These magnetic perturbations tend to repel field lines and as a result, the field lines near the light cylinder inflate to infinity and open up. In the vicinity of the light cylinder, the force-free condition is violated and dissipation effects and particle acceleration create electromagnetic emission detectable on Earth. 
The magnetosphere can then be divided into two regions with different properties (see Figure~\ref{fig:ch2_sketch_magnetosphere}). The magnetic field lines that do not cross the light cylinder form the so-called closed magnetosphere. Here the plasma is trapped and the condition $\boldsymbol{E} \cdot \boldsymbol{B} = 0$ is valid everywhere. This region should therefore be electromagnetically inactive as particle acceleration is suppressed.
The field lines that cross the light cylinder and are inflated to infinity form the open field line region. Here charges are free to stream along the magnetic field lines and escape to infinity. Therefore here the condition $\boldsymbol{E} \cdot \boldsymbol{B} = 0$ can be violated and gaps with low-density plasma can be created where charged particles are accelerated. The open field line region is therefore active and it is the region where electromagnetic emission from pulsars is believed to be produced. 

%=============================================================================

\section{Dipolar spin-down evolution} \label{sec:ch2_dip_spindown_evol}

The observation of the secular increase of spin periods for the detected neutron stars implies that they are losing rotational energy over time. Assuming that neutron stars are solid bodies the loss of rotational energy can be computed as:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_rotational_energy_loss}
    \frac{{\rm d} E_{\rm rot}}{{\rm d} t} &= \frac{{\rm d}}{{\rm d}t} \left( \frac{1}{2} I_{\rm NS} \omega^2 \right) = I_{\rm NS} \omega \frac{{\rm d} \omega}{{\rm d}t} = - 4 \pi^2 I_{\rm NS} \frac{{\rm d}P}{{\rm d}t} \frac{1}{P^3} \nonumber \\
                             & \simeq - \unit[4 \times 10^{31}]{erg \, s^{-1}} \left( \frac{\dot P}{\unit[10^{-15}]{s \, s^{-1}}} \right) \left( \frac{P}{\unit[1]{s}} \right)^{-3},
\end{align}
%--------------------------------------------------------------
where we assume a neutron star moment of inertia $I_{\rm NS} \simeq \unit[10^{45}]{g \, cm^2}$ which is constant in time. 

If a neutron star can be simply pictured as a rotating magnetic dipole with moment vector $\boldsymbol{\mu}$ misaligned by an angle $\chi$ with respect to the rotation axis, the spin-down can be explained using classical electrodynamics arguments \citep[see for example][]{Shapiro1983}.
In classical electrodynamics a rotating misaligned magnetic dipole emits electromagnetic energy \citep[see][]{Jackson1998}. In analogy with the Larmor formula for an accelerated charge, a time-varying magnetic dipole radiates away a total power integrated over the solid angle equal to: 
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_mag_dipole_radiation}
\frac{{\rm d} E}{{\rm d} t} = \frac{2}{3 c^3} \left| \frac{ {\rm d}^2 \boldsymbol{\mu}}{{\rm d}t^2} \right|^2.
\end{align}  
%-----------------------------------------------------------------
For a misaligned magnetic dipole with an inclination angle $\chi$, rotating at an angular frequency $\omega$, we can write the magnetic dipole moment components as a function of time $t$ in Cartesian coordinates. We assume rotation about the $z$ axis:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_mag_moment_cart}
\boldsymbol{\mu} = \mu \begin{bmatrix}
           \sin{\chi} \cos{\omega t} \\
           \sin{\chi} \sin{\omega t} \\
           \cos{\chi}
         \end{bmatrix}.
\end{align}  
%-----------------------------------------------------------------
where $\mu = |\boldsymbol{\mu}|$.
If we compute the second time derivative for this vector we find:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_2der_mag_moment_cart}
\frac{ {\rm d}^2 \boldsymbol{\mu}}{{\rm d}t^2} = \mu \begin{bmatrix}
           - \omega^2 \sin{\chi} \cos{\omega t} \\
           - \omega^2 \sin{\chi} \sin{\omega t} \\
           0
         \end{bmatrix}.
\end{align}  
%-----------------------------------------------------------------
Here we have assumed that the spin frequency, the magnetic moment and the inclination angle change on timescales much longer than a rotation period so that they can be assumed as constants in computing these derivatives, i.e., they do not explicitly depend on the time $t$.
By computing the squared module of the vector above and substituting it into Equation~\eqref{eq:ch2_mag_dipole_radiation} we get an emitted power:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_mag_dipole_radiation_2}
\frac{{\rm d} {E}}{{\rm d} t} = \frac{2 \mu^2}{3 c^3} \omega^4 \sin^2{\chi}. 
\end{align}  
%-----------------------------------------------------------------
By assuming that this electromagnetic energy is emitted at the expense of the rotational energy we can equate Equation~\eqref{eq:ch2_rotational_energy_loss} with Equation~\eqref{eq:ch2_mag_dipole_radiation_2} to obtain an equation that describes how the spin frequency changes in time:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_omegadot_vacuum}
    \frac{{\rm d} \omega}{{\rm d}t} = -\frac{2 \mu^2}{3 c^3 I_{\rm NS}} \omega^3 \sin^2{\chi}. 
\end{align}
%--------------------------------------------------------------
 
We find an analogous result by considering a more sophisticated calculation. By picturing the neutron star as a spherical conductor rotating in an electromagnetic field in vacuum it is possible to compute the net torque acting on it. In particular the electric and magnetic fields generate forces on the charges in the conductor which in turn generate a net torque acting on the conductor surface. This torque, $\boldsymbol{M}$, can be estimated by the following integral computed over the neutron star surface $S$ \citep[see][]{Michel1970, Philippov2014}: 
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_torque_em}
    \boldsymbol{M} = \int_S \boldsymbol{n} \cdot \left( \boldsymbol{r} \times \boldsymbol{T} \right) {\rm d} S,  
\end{align}
%--------------------------------------------------------------
where $\boldsymbol{r}$ is the radial vector originating in the neutron star centre, $\boldsymbol{T}$ is the Maxwell stress tensor and $\boldsymbol{n}$ is the unit vector perpendicular to the surface. By considering the expressions for the electromagnetic fields near the stellar surface computed by \cite{Deutsch1955} for a rotating star characterized as a misaligned magnetic dipole in vacuum, \cite{Michel1970} computed the non-vanishing torque components. The first one is antiparallel to the spin frequency vector and causes the neutron star to spin down:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_torque_em_parallel}
    M_{\parallel} =  - \frac{2 \mu^2}{3 c^3} \omega^3 \sin^2{\chi}. 
\end{align}
%--------------------------------------------------------------
The second one is perpendicular to the spin frequency vector and acts in the plane defined by the two vectors $\boldsymbol{\omega}$ and $\boldsymbol{\mu}$. While it does not change the spin frequency, it is responsible for the alignment of the magnetic axis with the rotational axis:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_torque_em_perpendicular}
    M_{\perp} =  - \frac{2 \mu^2}{3 c^3} \omega^3 \sin{\chi} \cos{\chi}.
\end{align}
%--------------------------------------------------------------
A third component is perpendicular to the $\boldsymbol{\omega} - \boldsymbol{\mu}$ plane and causes precession of the spin frequency vector around the magnetic axis \citep[][]{Philippov2014}. In the following, we will not take into account this precession since it does not affect the evolution of the spin period and inclination angle. 
The evolution of the angular momentum vector, $\boldsymbol{L}$ of the neutron star is then given by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_torque}
    \frac{{\rm d} \boldsymbol{L}}{{\rm d} t} = I_{\rm NS} \frac{{\rm d} \boldsymbol{\omega}}{{\rm d} t} = \boldsymbol{M},  
\end{align}
%--------------------------------------------------------------
which gives the following coupled differential equations:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_rot_evol_vacuum}
    \frac{{\rm d} \omega}{{\rm d} t} &= -\frac{2 \mu^2}{3 c^3 I_{\rm NS}} \omega^3 \sin^2{\chi}, \\
    \frac{{\rm d} \chi}{{\rm d} t} &= - \frac{2 \mu^2}{3 c^3 I_{\rm NS}} \omega^2 \sin{\chi} \cos{\chi}.
\end{align}
%--------------------------------------------------------------
Note that the first equation is the same as Equation~\eqref{eq:ch2_omegadot_vacuum}.
In general, neutron stars evolves towards longer periods and a configuration where the magnetic dipole axis is aligned with the rotation axis. Therefore rotational evolution tends towards a state where the energy losses due to the torques are minimized as can be seen from Equation~\eqref{eq:ch2_mag_dipole_radiation_2}. However, these equations are valid in the case of a vacuum magnetosphere which as we have seen in Section~\ref{sec:ch2_magnetosphere} is not the most realistic scenario.

For plasma-filled magnetospheres, an analytical solution of the torques can not be derived and simulations are required due to the non-linearity of the problem. Through 3D simulations of force-free plasma-filled magnetospheres \cite{Spitkovsky2006} found that the emitted electromagnetic luminosity can be well described by the following relation:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_pulsar_lum_forcefree}
\left( \frac{{\rm d} {E}}{{\rm d} t} \right)_{\rm force-free} = \frac{\mu^2}{c^3} \omega^4 (\kappa_0 + \kappa_1 \sin^2{\chi}). 
\end{align}  
%-----------------------------------------------------------------
The rotational evolution of a neutron star can then be approximated by the two following equations:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_rot_evol_forcefree}
\frac{{\rm d} \omega}{{\rm d} t} &=  - \frac{\mu^2}{c^3 I_{\rm NS}} \omega^3 \left( \kappa_0 + \kappa_1 \sin^2 \chi \right), \\
\frac{{\rm d} \chi}{{\rm d} t} &=  - \frac{\mu^2}{c^3 I_{\rm NS}} \omega^2 \left( \kappa_2 \sin\chi \cos\chi \right),
\end{align}  
%-----------------------------------------------------------------  
and substituting $\omega = 2\pi/P$ we get: 
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_rot_evol_forcefree_2}
    \frac{{\rm d} P}{{\rm d}t} &= \frac{ 4 \pi^2 \mu^2}{ c^3 I_{\rm NS} P } \left( \kappa_0 + \kappa_1 \sin^2 \chi \right), \\
    \frac{{\rm d} \chi}{{\rm d}t} &= - \frac{ 4 \pi^2 \mu^2}{ c^3 I_{\rm NS} P^2 } \left( \kappa_2 \sin\chi \cos\chi \right),
\end{align}
%--------------------------------------------------------------
The parameters $\kappa_0$, $\kappa_1$ and $\kappa_2$ are derived by fitting simulation results and for force-free magnetosphere they take the values $\kappa_0 \simeq \kappa_1 \simeq \kappa_2 \simeq 1$ \citep{Philippov2014}.
Compared to the vacuum solution (where $\kappa_0 = 0$, $\kappa_1 = 2/3$ and $\kappa_2 = 1$) the electromagnetic torque and the energy loss does not vanish when the magnetic dipole axis aligns with the rotation axis and the torque exerted on the star can be a factor $\sim 2$ stronger.

\subsection{Dipole magnetic field estimate}

By considering the magnetic dipole breaking model outlined above we can estimate the dipolar magnetic field of a neutron star from its timing properties $P$ and $\dot{P}$. 
If we consider the magnetic field strength at the magnetic pole of the neutron star at $r = R_{\rm NS}$, from Equation~\eqref{eq:ch2_B_dipole} we get the expression:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_mag_dipole_B_pole}
B_{\rm p} = \frac{2 \mu}{R_{\rm NS}^3} \; \Longrightarrow \; \mu = \frac{B_{\rm p} R_{\rm NS}^3}{2}.
\end{align}  
%-----------------------------------------------------------------
If we consider the magnetic field strength at the magnetic equator of the neutron star we get that it is half of the value at the magnetic pole:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_mag_dipole_B_equat}
B_{\rm e} = \frac{\mu}{R_{\rm NS}^3} \; \Longrightarrow \; \mu = B_{\rm e} R_{\rm NS}^3.
\end{align}  
%-----------------------------------------------------------------
We can substitute Equation~\eqref{eq:ch2_mag_dipole_B_pole} or Equation~\eqref{eq:ch2_mag_dipole_B_equat} into Equation~\eqref{eq:ch2_rot_evol_forcefree_2} to obtain a relation between the observed quantities $P$ and $\dot{P}$ and the magnetic field strength at the poles or at the equator.
In the literature, the vacuum magnetosphere model is often assumed even if less realistic. This usually implies an overestimation of the magnetic field strength by a factor of $\sim 2$ with respect to the force-free magnetosphere solution. By assuming for the sake of simplicity an inclination angle $\chi = \pi/2$ (since it is usually unknown) we obtain a formula to roughly estimate the strength of the magnetic field at the neutron star poles or equator as a function of the timing properties:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_Bpol_vacuum}
    B_{\rm p} = \left( \frac{ 3 c^3 }{ 2 \pi^2 } \frac{  I_{\rm NS} P \dot{P} }{R_{\rm NS}^6} \right)^{1/2} \simeq \unit[2 \times 10^{12}]{G} \left( \frac{P}{\unit[1]{s}} \right)^{1/2} \left( \frac{\dot{P}}{\unit[10^{-15}]{s \, s^{-1}}} \right)^{1/2},
\end{align}
%--------------------------------------------------------------
where we consider a neutron star moment of inertia $I_{\rm NS} \simeq \unit[10^{45}]{g \, cm^2}$ and radius $R_{\rm NS} \simeq \unit[10^6]{cm}$. Using this equation we can plot the lines of constant magnetic field in the $P-\dot{P}$ diagram (see Figure~\ref{fig:ch1_PPdot_diagram}).

\subsection{Characteristic age estimate}

By assuming that both the magnetic field and the inclination angle stay constant during the neutron star's life, one can integrate of Equation~\eqref{eq:ch2_rot_evol_forcefree} in time to obtain a characteristic age:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_characteristic_age}
    \tau_{\rm c} = -\frac{\omega^3}{2\dot{\omega}} \left( \frac{1}{\omega^2} - \frac{1}{\omega_0^2} \right), 
\end{align}
%--------------------------------------------------------------
where $\omega_0$ is the initial spin frequency and $\omega$ and $\dot{\omega}$ are the current values of spin frequency and spin frequency derivative.
If we assume that $\omega_0 \gg \omega$, which means that the neutron star was rotating much faster at birth than at the current time, Equation~\eqref{eq:ch2_characteristic_age} becomes:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_characteristic_age_approx}
    \tau_{\rm c} = -\frac{\omega}{2\dot{\omega}} = \frac{P}{2\dot{P}} \simeq \unit[1.6 \times 10^{7}]{yr} \left( \frac{P}{\unit[1]{s}} \right) \left( \frac{\dot{P}}{\unit[10^{-15}]{s \, s^{-1}}} \right)^{-1}.
\end{align}
%--------------------------------------------------------------
Using this equation we can plot the lines of constant characteristic age in the $P-\dot{P}$ diagram (see Figure~\ref{fig:ch1_PPdot_diagram}).

The characteristic age in general represents an upper limit on the true neutron star age. Indeed for very young pulsars the assumption that $\omega_0 \gg \omega$ could not hold as their spin period can be still very close to the value at birth. Furthermore, for older pulsars, if one takes into account that the magnetic field decays over time the characteristic age could exceed the real age of the neutron star by orders of magnitude. In these cases the characteristic age fails to give a good estimate for the actual age.
%--------------------------------------------------------------------------------------------

\section{Magnetic field evolution}  \label{sec:ch2_B_evol}

%----------------------------------------------------
\begin{figure*}
\includegraphics[width=0.47\textwidth]{Figures/Bfield_evol_anal.pdf}
\includegraphics[width=0.47\textwidth]{Figures/Bfield_evol_sim.pdf}
\caption[Dipolar magnetic field evolution curves]{Examples of dipolar magnetic field evolution curves. The analytical solution in Equation \eqref{eq:ch2_B_decay} (\textit{left panel}) is compared to the numerical solution from 2D magneto-thermal simulations \citep{Vigano2021} (\textit{right panel}). In the right panel, the purple curve corresponding to an initial magnetic field of $\unit[10^{12}]{G}$ appears truncated due to code constraints in modeling the micro-physical behaviour of the neutron-star crust at low temperatures.}
\label{fig:ch2_B_evolution}
\end{figure*}
%----------------------------------------------------

Much effort has been put into modeling the magnetic field geometry and evolution inside a neutron star. 
Soon after birth, a solid crust of about $\unit[1]{km}$ thickness is formed.
At the densities of the crust ($\unit[10^{10} - 10^{14}]{g \, cm^{-3}}$), matter is pressure-ionized. Atoms are so densely packed together that electrons are not bound to a single nucleus but feel the electric fields of all the neighbouring nuclei. As a consequence, while the ions in the lattice or the pasta phase layer (see Section~\ref{sec:ch1_internal_structure_MR_relation}) have very restricted mobility, electrons are free to flow constituting the main source of conductivity. Therefore describing the magnetic field evolution in the crust is more straightforward as the electrons are the only charged particles affecting it and the microphysical properties of matter are relatively well known. On the other hand, describing the field geometry and evolution in the liquid core is more complex. Due to the extreme conditions prevalent within the core, the exact composition and the properties of matter are still uncertain. In the fluid core, besides electrons, also neutrons, protons, muons and possibly more exotic particles could influence the magnetic field evolution. In particular it is believed that neutron superfluidity and proton superconductivity can play a critical role for the internal dynamics \citep[see for example][]{Chamel2017, Wood2022}. In general, for the core, it is very challenging to accurately incorporate realistic microphysics and estimate the impact of these effects on the magnetic field's evolution \citep{Vigano2021}. Here we will focus instead on the evolution of the magnetic field which is confined in the neutron star crust.
In general, the equation governing the magnetic field evolution is Maxwell's induction equation:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_induction_eq_short}
    \frac{\partial \boldsymbol{B}}{\partial t} = - c \left( \boldsymbol{\nabla} \times \boldsymbol{E} \right).
\end{align}
%--------------------------------------------------------------
For a conducting fluid of electrons, moving with velocity $\boldsymbol{v}_e$ and in the presence of a magnetic field $\boldsymbol{B}$, the electric field $\boldsymbol{E}$ is related to the current density $\boldsymbol{j}$ through the generalized Ohm's law:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_E_ohm_law}
    \boldsymbol{E} = \frac{\boldsymbol{j}}{\sigma_e} - \frac{\boldsymbol{v_e}}{c} \times \boldsymbol{B},
\end{align}
%--------------------------------------------------------------
where $\sigma_e$ is the electrical conductivity that can be defined in terms of the mean free time between collisions or relaxation time $\tau_e$ \citep{Longair2011}:
%--------------------------------------------------------------
\begin{align}
    \sigma_e = \frac{e^2 n_e \tau_e}{m_e}.
\end{align}
%--------------------------------------------------------------
The electron velocity is also related to the current and electron density $n_e$ trough:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_e_velocity}
    \boldsymbol{v}_e = - \frac{\boldsymbol{j}}{e n_e}.
\end{align}
%--------------------------------------------------------------
We can also assume that the timescale for collisions inside the plasma is much shorter than the timescale of the variation of the electromagnetic field so that we can neglect the displacement current term in Ampere's law and express the current density as:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_current_density}
    \boldsymbol{j} = - \frac{c}{4 \pi} \left( \boldsymbol{\nabla} \times \boldsymbol{B} \right).
\end{align}
%--------------------------------------------------------------
Therefore by combining the four equations above, the induction equation assumes the form \citep{Pons2007, Vigano2012}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_induction_eq}
    \frac{\partial \boldsymbol{B}}{\partial t} = - \boldsymbol{\nabla} \times \left( \frac{c^2}{4 \pi \sigma_e} \boldsymbol{\nabla} \times \boldsymbol{B} + \frac{c}{4 \pi e n_e} (\boldsymbol{\nabla} \times \boldsymbol{B}) \times \boldsymbol{B} \right).
\end{align}
%--------------------------------------------------------------

The first term in the parentheses describes the Ohmic dissipation. It is responsible for converting magnetic energy into heat according to $Q = j^2 / \sigma_e$ which is then deposited in the crust. In a neutron star crust, the conductivity $\sigma_e$ is dominated by the electronic transport and depends on the crustal temperature, the electron density, and the impurity concentration \textbf{should define the impurity parameter?}.
In general, for higher temperatures, and for larger impurity concentration the conductivity is lower as there is more scattering between the electrons and the lattice.
As a result the magnetic field evolution is highly coupled to the temperature evolution. The higher the magnetic field, the greater the dissipation and the heat deposited into the crust. In this way the stellar surface is kept hot for longer times. This in turn affects the microphysical properties of the crust and the electrical conductivity so that the heat deposition itself influences how the magnetic field dissipates.
Furthermore, the electron density varies over about four orders of magnitude in the crust. As a consequence, the electric conductivity varies by many orders of magnitude across the neutron star crust as well. What drives the evolution is usually the resistivity of the region where currents are predominantly placed. For example, the dissipation will be greater if currents are mainly circulating in the pasta layer of the crust. Here the transport properties are uncertain but the irregularities in the nuclear matter shapes and charge distribution should enhance the resistivity and therefore the magnetic field dissipation \citep{Horowitz2015, Nandi2018}.

The second part is a non-linear term which strongly depends on the magnetic field strength and is related to the Hall drift.  It does not cause dissipation, but it is responsible for the drift and rearrangement of the electric currents inside the crust and the redistribution of the magnetic energy on smaller scales. By affecting the distribution and scale of the electric currents the Hall effect is responsible of enhancing the Ohmic dissipation. As it depends only on the degenerate electron density it should be insensitive to temperature \citep[see also][]{Cumming2004}.

%The magnetic field geometry and evolution are also important to determine how and where the heat is deposited into the crust. Indeed the presence of the magnetic field makes the thermal conductivity anisotropic suppressing the heat transport across the magnetic field lines. This creates hot spots and inhomogeneities in the surface temperature distribution \citep{Gourgouliatos2018}.  

If one is concerned only with the evolution of the magnitude of the magnetic field in time, the induction equation can be rewritten in an approximated form as \citep[see][]{Aguilera2008b, Aguilera2008a}:
%-----------------------------------------------------------------
\begin{align}	\label{eq:ch2_Bdot}
\frac{{\rm d} B}{{\rm d} t} &\simeq - \frac{c^2 B}{4 \pi \sigma L^2} - \frac{c B^2}{4 \pi e n_e L^2} \\ \nonumber
                &= - \frac{B}{\tau_{\rm Ohm}} - \frac{B^2}{B_0 \tau_{\rm Hall,0}},
\end{align}  
%-----------------------------------------------------------------      
where the spatial derivatives have been replaced by a factor $1/L$ where $L$ is a typical length scale over which the physical quantities $B$, $n_e$ and $\sigma_e$ change. We can also define two typical timescales, one for the Ohmic dissipation, and the other for the Hall drift:
%----------------------------------------------------
\begin{align} \nonumber
    \tau_{\rm Hall,0} &= \frac{4 \pi e n_e L^2}{c B_0} \\ 
    &\simeq \unit[6.4 \times 10^4]{yr} \left( \frac{n_e}{\unit[10^{35}]{cm^{-3}}} \right)
    \left( \frac{L}{\unit[1]{km}} \right)^2 
    \left( \frac{B_0}{\unit[10^{14}]{G}} \right)^{-1}, 
        \label{eq:ch2_tau_hall} \\
    \tau_{\rm Ohm} &= \frac{4 \pi \sigma L^2}{c^2} \nonumber \\ 
    &\simeq \unit[4.4 \times 10^6]{yr} \left( \frac{\sigma}{\unit[10^{24}]{s^{-1}}} \right)
    \left( \frac{L}{\unit[1]{km}} \right)^2, 
        \label{eq:ch2_tau_ohm}
\end{align}
%----------------------------------------------------    
where the numerical values are taken from \cite{Cumming2004}. Note that the Hall timescale defined here is inversely proportional to the initial magnetic field magnitude $B_0$. 
By neglecting the influence of the temperature we find the following analytical solution for Equation~\eqref{eq:ch2_Bdot}:
%----------------------------------------------------
\begin{align}
    B(t) = B_0 \frac{e^{-t/\tau_{\rm Ohm}}}{1 + \frac{\tau_{\rm Ohm}}{\tau_{\rm Hall,0}} \left[ 1 - e^{-t/\tau_{\rm Ohm}} \right]}. 
        \label{eq:ch2_B_decay}
\end{align}
%----------------------------------------------------
Even if it is a very crude approximation, this equation captures a first stage that is characterized by rapid (non-exponential) decay regulated by the Hall timescale $\tau_{\rm Hall,0}$, and a second stage that is characterized by exponential decay due to Ohmic dissipation and regulated by the timescale $\tau_{\rm Ohm}$ (see left panel in Figure~\ref{fig:ch2_B_evolution}).

To model the magnetic field evolution and decay in neutron stars consistently, a complete magneto-thermal simulation is required that takes into account the coupled magnetic field and temperature evolution. Moreover inside the neutron star general relativistic effects become relevant. Therefore the induction equation \eqref{eq:ch2_induction_eq} has to be corrected to take into account the curvature of space-time. Generally the shwarzschild static metric is sufficient as any deformation induced by rotation and the magnetic fields are negligible. In recent years numerical codes able to simulate the magnetic field and temperature evolution of neutron stars have been developed. In particular large efforts have been put into 2D axis-symmetric simulations \citep[see for example][]{Aguilera2008a, Pons2009, Vigano2012, Vigano2021}. More recently the more complex but more realistic 3D case is being explored \citep[see][]{Gourgouliatos2016, DeGrandis2020, Dehman2023}. The right panel of Figure~\ref{fig:ch2_B_evolution} shows the magnetic field evolution curves predicted by 2D magneto-thermal simulations \citep{Vigano2021}.

%--------------------------------------------------------------------------------------------

\section{Pulsar radio emission} \label{sec:ch2_radio_em_geometry}

As we have described in Section~\ref{sec:ch2_magnetosphere}, the magnetosphere surrounding a neutron star is divided into a closed field line and an open field line region. According to the standard theory \citep{Goldreich1969, Sturrock1971, Ruderman1975}, in the open field line region particles can freely stream along the field lines. If charges are not continuously extracted from the surface the outflow of particles eventually generates vacuum or low-density regions, so-called plasma gaps, above the magnetic poles. Inside these gaps the force-free condition $\boldsymbol{E} \cdot \boldsymbol{B} = 0$ can be violated as the electric field parallel to the magnetic field lines is not perfectly screened anymore. New particles can therefore be extracted from the stellar surface and accelerated up to relativistic speed leading to an avalanche of pair production. The mechanism producing the radio emission in pulsars is not well understood, but it is believed that in this process bunches of $e^+ \, e^-$ pairs produced in the gap oscillate coherently to produce radio emission at a certain distance from the polar cap see Section~\ref{sec:ch2_radio_em_deathlines}. 

\subsection{The polar cap model and radio emission geometry}

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{polar_cap_geometry.pdf}
\caption[Geometry of the polar cap]{Sketch showing the geometry of the polar cap emission model for an aligned rotator. The polar cap region is delimited by the last closed field lines extending to the light cylinder. A magnetic field line can be parameterised as curve described by the coordinates $r$ and $\theta$ (see text for more details). }
\label{fig:ch2_polar_cap}
\end{figure*}
%----------------------------------------------------

The common picture is that this radio emission is generated in conical beams delimited by the open field lines around the magnetic poles. 
We can estimate the size of these conical beams by considering the size of the polar caps where the open field lines are anchored to the neutron star. The polar cap size depends on the amount of field lines that are opened which in turn depends on the size of the light cylinder (see Equation~\eqref{eq:ch2_light_cylinder}, i.e., on the spin period of the neutron star. To see this consider Figure~\ref{fig:ch2_polar_cap} showing a sketch of a neutron star with the magnetic dipole moment aligned to the rotation axis of the star. 
We parametrize a magnetic field line as a curve $\boldsymbol{r} = r(\theta) \hat{\boldsymbol{e}_r}$ in space, where $\theta$ is the angle between the rotation axis and the vector $\boldsymbol{r}$ whose origin is located in the star's center and pointing to a random position on the field line. The magnetic field vector $\boldsymbol{B}$ is therefore proportional to the tangent vector of the curve given by $d\boldsymbol{r}/d\theta = (dr/d\theta) \hat{\boldsymbol{e}_r} + r \hat{\boldsymbol{e}_{\theta}}$.
By considering the expression of the magnetic dipole in spherical coordinates (Equation~\eqref{eq:ch2_B_dipole_sph_coord}) we obtain the following equations:
%--------------------------------------------------------------
\begin{align}
    \frac{{\rm d} r}{{\rm d}\theta} &= \lambda(\theta) \frac{\mu}{r^3} 2 \cos(\theta), \\
                     r &= \lambda(\theta) \frac{\mu}{r^3} \sin(\theta), 
\end{align}
%--------------------------------------------------------------
where $\lambda(\theta)$ represents a generic proportionality coefficient.
If we consider the ratio between these two equations we end up with the following differential equation:
%--------------------------------------------------------------
\begin{align}
    \frac{{\rm d} r}{r {\rm d}\theta} = \frac{2\cos{\theta}}{\sin{\theta}}. 
\end{align}
%--------------------------------------------------------------
We consider the last closed field line that delimits the polar cap region and is tangent to the light cylinder. The equation above can be integrated from a generic radius $r$ corresponding to a generic $\theta$ to the light cylinder radius $r = r_{\rm LC}$ corresponding to $\theta = \pi/2$:
%--------------------------------------------------------------
\begin{align}
    \int_{r}^{r_{\rm LC}} \frac{{\rm d} r'}{r'} = \int_{\theta}^{\pi/2} \frac{2\cos{\theta'}}{\sin{\theta'}} d\theta' \; \Longrightarrow \;
           \ln{\frac{r_{\rm LC}}{r}} = 2\ln{\frac{1}{\sin{\theta}}}. \\ \nonumber
\end{align}
%--------------------------------------------------------------
This implies:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_const_Bline}
    \frac{\sin^2{\theta}}{r} = \frac{1}{r_{\rm LC}}.
\end{align}
%--------------------------------------------------------------
Generally the quantity $\sin^2{\theta}/r$ is constant along any dipolar field line.
With this relation, by setting $r = R_{\rm NS}$ we can find the angular radius of the polar cap on the neutron star surface:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_polar_cap_angular_radius}
    \sin{\theta_{\rm pc}} &= \left( \frac{R_{\rm NS}}{r_{\rm LC}} \right)^{1/2} \\
    \Longrightarrow \; \theta_{\rm pc} \sim \left( \frac{2 \pi R_{\rm NS}}{cP} \right)^{\frac{1}{2}} &= \unit[0.015]{rad} \, [\unit[0.87]{deg}] \left( \frac{R_{\rm NS}}{\unit[11]{km}} \right) \left( \frac{P}{\unit[1]{s}} \right)^{-1/2},
\end{align}
%--------------------------------------------------------------
where we assumed that the the polar cap angular aperture is small i.e., $\theta_{\rm pc} \lesssim 30^{\circ}$ \citep{Lorimer2012}.

We now consider an emission point on a field line at the edge of the polar cap, with coordinates $(r_{\rm em}, \, \theta_{\rm em})$. By using Equation~\eqref{eq:ch2_const_Bline} we can write:
%--------------------------------------------------------------
\begin{align}
    \sin{\theta_{\rm em}} = \left( \frac{r_{\rm em}}{r_{\rm LC}} \right)^{1/2} \; \Longrightarrow \;
    \theta_{\rm em} \sim \left( \frac{2 \pi r_{\rm em}}{cP} \right)^{1/2},
\end{align}
%--------------------------------------------------------------
where we have assumed again that the polar cap region is narrow and the emission point is close to the magnetic axis, i.e., $\theta_{\rm em} \lesssim 30^{\circ}$. As the field lines are curved, the opening angle $\rho_{\rm em}$ of the emission cone tangent to the field lines at the polar coordinates $(r_{\rm em}, \, \theta_{\rm em})$ is generally a little bigger than the polar angle $\theta_{\rm em}$. The relation between these two angles was found by \cite{Gangadhara2001}, and for small angles reduces to:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_beam_angular_aperture}
    \rho_{\rm em} \sim \frac{3}{2} \theta_{\rm em} \sim \left( \frac{9 \pi r_{\rm em}}{2 cP} \right)^{\frac{1}{2}} = \unit[0.069]{rad} \, [\unit[3.95]{deg}] \left( \frac{r_{\rm em}}{\unit[100]{km}} \right)^{1/2} \left( \frac{P}{\unit[1]{s}} \right)^{-1/2}.
\end{align}
%--------------------------------------------------------------
This gives the half-opening angle of the radio emission cone at the two magnetic polar regions of the neutron star. The modifications arising by taking into account a misaligned magnetic dipole moment and general relativistic effects are small and in general can be neglected \citep{Kapoor1998}.

\subsection{Pulse width}

%-------------------------------------------------------------
\begin{figure}[t!]
\centering
\includegraphics[width = 0.8\textwidth]{Figures/radio_beam_geometry.pdf}
\caption[Radio beam geometry]{\label{fig:ch2_radio_beam_geometry}{Radio beam geometry. The magnetic dipole moment $\boldsymbol{\mu}$ is misaligned by an angle $\chi$ with respect to the rotation axis defined by $\boldsymbol{\omega}$. The line of sight cuts the emission cone at an angle $\beta$ relative to the centre of the beam. The angular pulse width is given by $\varphi$.}}
\end{figure}  
%-------------------------------------------------------------
%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{W-P_relation.pdf}
\caption[Pulse widths versus spin period relation]{Plot of pulse-widths $w_{50}$ measured at the 50\% of the maximum pulse amplitude versus the spin period $P$ for 1450 normal pulsars detected at 1.4 GHz (excluding millisecond and other recycled pulsars) from the ATNF database \citep{Manchester2005}. We also include 21 cases of pulsars being almost orthogonal rotators and manifesting inter-pulses due to our line of sight crossing both magnetic poles (red dots) and 11 cases of almost aligned pulsars where only one magnetic pole is visible but manifesting interpulses (green dots). The black solid line represents the fit of the orthogonal-rotator pulsars (red dots) \citep[see][for more details]{Maciesiak2011b, Maciesiak2012} \citep[Figure taken from][]{Maciesiak2012}.}
\label{fig:ch2_w_P_relation}
\end{figure*}
%----------------------------------------------------
As the neutron star rotates, a pulse of radiation can be detected if our line of sight cuts through at least one of the radio beams. Therefore the features of the observed pulses depend on the geometry of the radio beam and the relative position at which the line of sight intercepts it.
Having computed the angular aperture of the radio beam $\rho_{\rm em}$ \eqref{eq:ch2_beam_angular_aperture}, we can now set up a relation that links it to the intrinsic pulse half-width $\varphi$ (expressed in radians) that an observer sees. We provide Figure~\ref{fig:ch2_radio_beam_geometry}, valid for a generic inclined rotator with $\chi$ the inclination angle between the magnetic dipole moment and the rotation axis, as a reference. Let's assume that as the star rotates our the line of sight intercepts the beam at an angular distance $\beta$ from its center. By assuming a sphere of unit radius, and considering the spherical triangle with sides $\chi + \beta$, $\chi$ and $\rho_{\rm em}$ we use the haversine law to write down the following relation:
%--------------------------------------------------------------
\begin{align}
    {\rm hav}\left( \rho_{\rm em} \right) =  {\rm hav}\left( \chi + \beta - \chi \right) + \sin \left( \chi + \beta \right) \sin \left( \chi \right) {\rm hav}\left( \varphi\right),
\end{align}
%--------------------------------------------------------------
where in general given an angle $\alpha$ the haversine function is defined as ${\rm hav}\left( \alpha \right) = \sin^2 \left( \alpha/2 \right)$. 
Solving for the square sine of the half pulse width, we can write the following formula \citep[see][]{Maciesiak2011a}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_radio_pulse_width}
    \sin^2 \left( \frac{\varphi}{2} \right) &=  \frac{\sin^2\left( \frac{\rho_{\rm em}}{2} \right) - \sin^2\left( \frac{\beta}{2} \right)}{\sin \left( \chi+\beta \right) \sin\left( \chi \right)} \\ \Longrightarrow \;
    \varphi &= 2 \arcsin{ \sqrt{ \frac{\sin^2\left( \frac{\rho_{\rm em}}{2} \right) - \sin^2\left( \frac{\beta}{2} \right)}{\sin \left( \chi+\beta \right) \sin\left( \chi \right)} }}.
\end{align} 
%--------------------------------------------------------------

To find the pulse width in time units we have to re-normalize for the spin period:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_pulse_width}
    w &= 2 \varphi \frac{P}{2 \pi} = 2 \frac{P}{\pi} \arcsin{ \sqrt{ \frac{\sin^2\left( \frac{\rho_{\rm em}}{2} \right) - \sin^2\left( \frac{\beta}{2} \right)}{\sin \left( \chi+\beta \right) \sin\left( \chi \right)} }}.
\end{align} 
%--------------------------------------------------------------

A simplified formula for the pulse width can be found if one assumes that the line of sight intercepts the radio beam in its centre (i.e. with $\beta = 0$) and that $\rho_{\rm em}$ and $\varphi$ are small ($\lesssim 30^{\circ}$). In this case we can approximate the relation in Equation~\eqref{eq:ch2_radio_pulse_width} as:
%--------------------------------------------------------------
\begin{align}
    \left( \frac{\varphi}{2} \right)^2 \sim  \frac{\left( \frac{\rho_{\rm em}}{2} \right)^2}{\sin^2 \left( \chi \right) }
    \Longrightarrow \; \varphi \sim \frac{\rho_{\rm em}}{\sin \left( \chi \right) },
\end{align}
%--------------------------------------------------------------
which leads to:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_pulse_width_simpli}
    w &= 2 \varphi \frac{P}{2 \pi} \sim 2 \frac{\rho_{\rm em}}{\sin{\chi}} \frac{P}{2 \pi} \sim \frac{2}{\sin{\chi}} \left( \frac{r_{\rm em} P}{2 \pi c} \right)^{\frac{1}{2}} \\ &\simeq \frac{\unit[0.015]{s}}{\sin{\chi}} \left( \frac{r_{\rm em}}{\unit[100]{km}} \right)^{1/2} \left( \frac{P}{\unit[1]{s}} \right)^{1/2}.
\end{align}
%--------------------------------------------------------------
Note that the $\sin{\chi}$ term corrects for the inclination angle. As the inclination angle decrease the observed pulse width increase even if the angular aperture $\rho_{\rm em}$ of the emission cone remains constant. This explain why in Figure~\ref{fig:ch2_w_P_relation} the orthogonal rotators are found at the extreme bottom part of the diagram and more aligned rotators are scattered above depending on the inclination angle. For example, if we observe an aligned rotator ($\chi \sim 0^{\circ}$) we do not see pulsed emission since our line of sight is always inside the radio beam. In this case, according to the formula above the pulse width goes to $\infty$ but this simply indicates that we are seeing continuous emission from the polar cap. 
Furthermore, as $-\rho_{\rm em} < \beta < \rho_{\rm em}$, the angle $\chi + \beta$ could become negative. This occur only when $\rho_{\rm em} > \chi$, and in that case it happens that the line of sight is always inside the beam and therefore also in this case no pulsation is observed. Some periodic modulation in the observed pulse profile can be still observed if the intensity profile of the beam is not uniform. 

To obtain an estimate of the emission cone aperture $\rho_{\rm em}$ from the pulse width $w$ measurements one can in principle use Equation~\eqref{eq:ch2_pulse_width}. However, deriving an estimate of the intrinsic pulse width $w$ is not always trivial. The observed pulse width usually differ from the intrinsic pulse width due to pulse broadening as the radio waves propagates through the interstellar medium (see Section~\ref{sec:ch2_detection}). Furthermore Pulsars exhibit different pulse profiles and widths due to various intrinsic properties, including magnetospheric dynamics, emission processes, and rotational irregularities. These differences make it challenging to predict or measure the pulse width accurately, especially for pulsars with complex emission patterns \citep[see][]{Lorimer2012}. Furthermore, we generally lack information on the relative angular position between the rotation axis, magnetic axis and line of sight.
For more details see also Chapter 3 in \cite{Lorimer2012}.

Overall even if this theoretical picture does not take into account all the complexity that might arise in reality, it predicts a relation $\rho_{\rm em} \sim P^{-1/2}$ which has been observed for samples of pulsars with reliable measurements of the pulse width \citep[see Figure~\ref{fig:ch2_w_P_relation} and][]{Rankin1993, Maciesiak2011b, Maciesiak2012}.
By using a sample of pulsars observed by the Parkes Murriyang radio telescope \cite{Johnston2019} found a shallower relation $\rho_{\rm em} \sim P^{-0.3}$. However the scatter of data in the pulse width - spin period plane is large and is partly produced by the unknown magnetic inclination angle $\chi$ as can be seen from Equation~\eqref{eq:ch2_pulse_width_simpli}. As $\chi$ is unknown, its effect is difficult to take into account and affects the correlation between these quantities. This work also suggests that a narrow range of emission heights $r_{\rm em}$ between around $\unit[200]{km}$ and $\unit[400]{km}$ seems to be preferred. 

%========================================================================

\subsection{Radio emission mechanism and radio death valley} \label{sec:ch2_radio_em_deathlines}

%----------------------------------------------------
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/death_lines.pdf}
\caption[Radio emission death valley]{Radio emission death valley delimited by the two extreme death lines (\textit{dashed lines}) defined in Equations~\eqref{eq:ch2_death_line_1} for a pure dipole configuration, and~\eqref{eq:ch2_death_line_2} for a twisted multipole configuration, respectively. The dots represent the observed radio pulsars from the ATNF catalog \citep{Manchester2005}, where the dipolar magnetic field values are estimated from the timing properties ($P$ and $\dot{P}$) using Equation~\ref{eq:ch2_Bpol_vacuum}.}
\label{fig:ch2_death_lines}
\end{figure*}
%----------------------------------------------------

If a gap devoid of plasma is formed above the polar cap region an electric potential difference is generated along a magnetic field line. Following \cite{Ruderman1975} we can consider a narrow gap above the polar region extending from the neutron star surface up to a height $H$.
A given potential difference $\Delta V$ will accelerate an electron (or a positron) up to an energy $\gamma m_e c^2 = e \Delta V$ which implies a Lorentz factor of:
%--------------------------------------------------------------
\begin{align}
    \gamma = \frac{e \Delta V} {m_e c^2}.
\end{align}
%--------------------------------------------------------------
By moving along the curved field lines the electron will emit curvature photons of energy \citep{Jackson1998}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_curv_photon_energy}
    h \nu = \frac{3}{4 \pi} \frac{h c}{r_{\rm c}} \gamma^3 = \frac{3}{4 \pi} \frac{h c}{r_{\rm c}} \left( \frac{e \Delta V}{m_e c^2} \right)^3,
\end{align}
%--------------------------------------------------------------
where $h$ is the Planck constant, $\nu$ is the photon frequency and $r_{\rm c}$ denots the curvature radius of the magnetic field line.
The condition that such a curvature photon with energy $h \nu > 2 m_e c^2$ moving through a magnetic field produces an electron-positron pair inside the gap is given by \citep[see][]{Ruderman1975, Chen1993}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_pair_creation_lim}
    \frac{h \nu}{2 m_e c^2} \frac{B_{\perp}}{B_{\rm QED}} \sim \frac{1}{15}.
\end{align}
%--------------------------------------------------------------
Here $B_{\rm QED} = 2 \pi m_e^2 c^3 / (e h)$ is the Schwinger magnetic field, defined as the magnetic field strength for which a cyclotron photon emitted by an electron gyrating around a field line will have an energy equal to $m_e c^2$.
$B_{\perp}$ is the component of the magnetic field perpendicular to the direction of propagation of the photon. Due to relativistic beaming the curvature photons are emitted along the direction of motion of the electron, i.e., almost parallel to the magnetic field lines, within an angle $\sim 1/\gamma$. Suppose that a curvature photon is emitted close to the stellar surface, where the magnetic field strength is $B_{\rm s}$. As the photon propagate inside the gap the component $B_{\perp}$ will grow up to an approximate maximum value given by $B_{\perp} \sim \frac{H}{r_{\rm c}} B_{\rm s}$. With all these considerations we can substitute Equation~\eqref{eq:ch2_curv_photon_energy} into Equation~\eqref{eq:ch2_pair_creation_lim} to find the relation:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_pair_creation_lim_2}
    \frac{3}{8 \pi} \left( \frac{e \Delta V} {m_e c^2} \right)^3 \frac{h}{m_e c} \frac{H}{r_{\rm c}^2} \frac{B_{\rm s}}{B_{\rm QED}} \sim \frac{1}{15}.
\end{align}
%--------------------------------------------------------------
This equation defines the minimum potential difference that is required to trigger a pair cascade inside the gap. According to the standard theory if a neutron star is not able to generate such electric potential difference in its magnetosphere it cannot be visible as a radio pulsar. On the other hand, triggering the pair cascade will also limit any further growth of $\Delta V$ above the value established by Equation~\eqref{eq:ch2_pair_creation_lim_2} as the produced plasma will progressively screen the electric field.

Assuming an aligned dipolar configuration for the magnetic field, due to the unipolar induction mechanism (see Section~\ref{sec:ch2_magnetosphere}), the maximum potential difference that can be generated along an open field line in the magnetosphere is given by the difference between the electric potential on the stellar surface given by Equation~\eqref{eq:ch2_unipolar_potential}) and the electric potential of the interstellar medium to which the open field line is connected at infinity. The interstellar electric potential can be assumed to vanish. From Equation~\eqref{eq:ch2_unipolar_potential}, the maximum potential difference can be established on the last open field line at the edge of the polar cap, i.e. at a coordinate $\theta = \theta_{\rm pc}$. By assuming $V_{\rm p} = 0$ we have:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_electric_potential_max}
    \Delta V_{\rm max} \simeq \frac{\omega \mu \sin^2{\theta_{\rm pc}}}{2 R_{\rm NS} c} = \frac{\omega B_{\rm p} R_{\rm NS}^2 \sin^2{\theta_{\rm pc}}}{2 c} = \frac{\omega^2 B_{\rm p} R_{\rm NS}^3}{2 c^2}.
\end{align}
%--------------------------------------------------------------
where we used Equation~\eqref{eq:ch2_mag_dipole_B_pole} and used the relation \eqref{eq:ch2_polar_cap_angular_radius}.
%This is indeed the potential difference between the polar magnetic field line and the last open field line at the edge of the polar cap.
This maximum potential difference depends solely on the dipole component of the field as it is the one determining the open field line configuration at large distance from the stellar surface, and is valid even if multipoles dominate near the stellar surface \citep{Ruderman1975}.
If the maximum potential difference $\Delta V_{\rm max}$ that can be produced in the magnetosphere is lower than the threshold defined by Equation~\eqref{eq:ch2_pair_creation_lim_2} the pair cascade can not be triggered and the neutron star is expected to be radio quiet. Therefore a necessary condition that has to be satisfied to turn on the radio emission is the following:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_death_line}
    \frac{3}{8 \pi} \left( \frac{e \Delta V_{\rm max}} {m_e c^2} \right)^3 \frac{h}{m_e c} \frac{H}{r_{\rm c}^2} \frac{B_{\rm s}}{B_{\rm QED}} \gtrsim \frac{1}{15}
\end{align}
%--------------------------------------------------------------
Depending on the assumptions that one makes on the magnetic field configuration near the surface and the gap geometry, that is the values of $B_{\rm s}$, $r_{\rm c}$ and $H$, the condition \eqref{eq:ch2_death_line} defines a threshold for the turning on and off of the radio emission in a pulsar. As the suppression of the radio emission depends on the particular magnetospheric properties of each pulsar, relation \eqref{eq:ch2_death_line} defines a "death valley" for the radio pulsars \citep[see][]{Chen1993}.
We can consider two extreme cases. For an ideal case of a pure dipole configuration we consider $B_{\rm s} = B_{\rm p}$, the curvature radius for an open field line can be approximated as $r_{\rm c} \sim r_{\rm LC} \sin{\theta_{\rm pc}} = (R_{\rm NS} r_{\rm LC})^{1/2}$ and the gap height can be taken to be equal to the polar cap radius $H \sim R_{\rm NS} \sin{\theta_{\rm pc}} = R_{\rm NS} \left( \frac{R_{\rm NS}}{r_{\rm LC}} \right)^{1/2}$ \citep{Chen1993}.
With these order of magnitude assumptions the following condition for the radio emission turning on is derived from Equation~\eqref{eq:ch2_death_line}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_death_line_1}
   B_{\rm p} \gtrsim \unit[2.0 \times 10^{12}]{G} \left( \frac{R_{\rm NS}}{\unit[10^6]{cm}} \right)^{-19/8} \left( \frac{P}{\unit[1]{s}} \right)^{15/8}.
\end{align}
%--------------------------------------------------------------
If instead multipoles dominate the magnetic field configuration near the surface, the value $B_{\rm s}$ could exceed the one of a pure dipole. We can introduce the parameterization $B_{\rm s} = b B_{\rm p}$ where $b$ is a numerical factor that takes into account deviations from the dipolar field value. Furthermore the curvature radius $r_{\rm c}$ in general scales inversely with the multiple order. We can consider an extreme case where the magnetic field near the surface is very twisted for the presence of strong multipole components. In this case for example we can assume $r_{\rm c} \sim H \sim R_{\rm NS}$. 
In this case, the condition for the radio emission becomes:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_death_line_2}
   B_{\rm p} \gtrsim \unit[8.3 \times 10^{10}]{G} \, b^{-1/4} \left( \frac{R_{\rm NS}}{\unit[10^6]{cm}} \right)^{-2} \left( \frac{P}{\unit[1]{s}} \right)^{3/2}.
\end{align}
%--------------------------------------------------------------
Given a neutron star with a spin period $P$, Equation~\eqref{eq:ch2_death_line_1} and \eqref{eq:ch2_death_line_2} give the minimum polar magnetic field strength that the star should have to trigger the radio emission.
Neutron stars with a lower magnetic field are considered radio-dead (see bottom right corner in Figure~\ref{fig:ch2_death_lines}).

\subsection{Energetics}

As we have seen in Section~\ref{sec:ch2_magnetosphere} and Section~\ref{sec:ch2_dip_spindown_evol}, a neutron star behaves as a unipolar inductor and spins down due to magnetic dipole breaking. It converts its rotational kinetic energy into electrical potential energy that ultimately leads to particle acceleration and electromagnetic emission.
The rate of loss of rotational energy is given by Equation~\eqref{eq:ch2_rotational_energy_loss}. This represents the total budget of rotational power that can be converted into electromagnetic power by the unipolar inductor process. As the potential difference that is established inside the magnetosphere is created at the expense of the rotational energy we expect a relation between the maximum potential difference and the rotational energy loss rate.
By expressing the polar magnetic field strength in Equation~\eqref{eq:ch2_electric_potential_max} as a function of the timing properties $P$ and $\dot{P}$ through Equation~\eqref{eq:ch2_Bpol_vacuum} the maximum potential difference inside the magnetosphere can be expressed as:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_electric_potential_max_2}
    \Delta V_{\rm max} \simeq \left( \frac{3}{2c} \frac{{\rm d} E_{\rm rot}}{{\rm d}t} \right)^{1/2}.
\end{align}
%--------------------------------------------------------------
We neglect the effect of the inclination angle which gives a correction of a factor 2 at most. 
The energy of the particles accelerated by this potential is given by $e \Delta V_{\rm max}$. This is the amount of energy that each particle can radiate away in the form of electromagnetic radiation.
Therefore the rotational energy is first converted into electrical potential energy which leads to particle acceleration and ultimately is radiated away in the form of electromagnetic radiation.
From this arguments it is reasonable to assume a link between the radio luminosity and the spin-down power. We consider a generic power-law dependence of the intrinsic radio luminosity $L$ of a pulsar on the rotational energy loss rate as:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_luminosity_Erot}
    L = L_{0} \left( \frac{\dot{E}_{\rm rot}}{\dot{E}_{\rm rot,0}} \right)^{\epsilon} = \mathcal{L}_{0} \left( \frac{\dot{P}}{P^3} \right)^{\epsilon},
\end{align}
%--------------------------------------------------------------
where $L_0$ is the luminosity at the reference rotational power $\dot{E}_{\rm rot,0}$ and:
%--------------------------------------------------------------
\begin{align} 
    \mathcal{L}_0 = L_0 \left( \frac{4 \pi^2 I_{\rm NS}}{\dot{E}_{\rm rot,0}} \right)^{\epsilon}.
\end{align}
%--------------------------------------------------------------
Considering a typical pulsar radio luminosity $L_0 \sim 10^{29}$ erg s$^{-1}$ corresponding to $\dot{E}_{\rm rot,0} = 10^{30}$ erg s$^{-1}$ \citep[see][]{Szary2014}, $\epsilon = 0.5$ and default values for the moment of inertia of a neutron star $I_{\rm NS} \sim 10^{45}$ g cm$^2$, we obtain $\mathcal{L}_0 \sim 3 \times 10^{35}$.
As the pulsar spins down it converts part of the rotational power in the form of radio waves. As the radio luminosity should not exceed the spin-down energy loss rate we can also express the equation above in terms of an efficiency $\eta$:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_luminosity_efficiency}
    L & = \eta(\dot{E}_{\rm rot}) \dot{E}_{\rm rot}.
\end{align}
%--------------------------------------------------------------
The efficiency is a function of the rotational power itself and in principle should not exceed 1.
Equation~\eqref{eq:ch2_luminosity_Erot} represents the intrinsic total radio luminosity emitted by the two radiation beams. This intrinsic luminosity is however difficult to derive from observations and instead, a pseudo-luminosity is usually estimated as we will discuss in Section~\ref{sec:ch2_pseudo_luminosity}. 

%=======================================================================

\section{Pulse propagation in the interstellar medium and detection} \label{sec:ch2_detection}

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{YMW17_model.pdf}
\caption[Galactic electron density for the YMW16 model]{Electron density in the Galactic plane ($z = 0$) for the YMW16 model \citep{Yao2017}. The Galactic Center is at the origin and the Sun is at $x = 0$, $y = \unit[8.5]{kpc}$. The dense annulus of central radius 4 kpc represents the Galactic molecular ring. Spiral arms have a pre-determined logarithmic spiral form and generally decay exponentially at large Galactocentric radii.
Exceptions are in the Carina and Sagittarius arms where there are over-dense and under-dense regions in Carina and Sagittarius
respectively. The Gum Nebula and Local Bubble features are faintly visible near the position of the Sun \citep[see][for more details]{Yao2017} \citep[Figure taken from][]{Yao2017}.}
\label{fig:ch2_e_density_model}
\end{figure*}
%----------------------------------------------------

The intensity, shape and duration of a detected radio pulse are influenced by a variety of factors which depend on both the propagation in the interstellar medium and instrumental effects. In the following I will discuss these aspects individually. 

Suppose that a pulsar with spin period $P$ and emitting two beams with an intrinsic radio luminosity $L$ is located at a distance $d$ from Earth. If the radio signal from this pulsar were to travel in complete vacuum, the pulse of radiation would have a width $w$ given by Equation~\eqref{eq:ch2_radio_pulse_width} and the flux of radiation reaching the Earth would be:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_radio_flux}
    S = \frac{L}{\Omega_{\rm em} d^2}.
\end{align}
%--------------------------------------------------------------
Here $\Omega_{\rm em}$ is the total solid angle covered by the two beams which are given by \citep[see][]{Lorimer2012}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_solid_angle}
    \nonumber \Omega_{\rm em}  & = 2 \times 2 \pi \int_{0}^{\rho_{\rm em}} \sin{\rho} {\rm d} \rho \\ \nonumber
       & = 4 \pi \left( 1 - \cos{\rho_{\rm em}} \right) \\
       & = 8 \pi \sin^2 \left( \frac{\rho_{\rm em}}{2} \right).
\end{align}
%--------------------------------------------------------------
The factor 2 is becuase we have two radio beams corresponding to each magnetic pole. In the last step we used the trigonometric identity $\left( 1 - \cos{\rho_{\rm em}} \right) = 2 \sin^2 \left( \frac{\rho_{\rm em}}{2} \right)$.

Radio telescopes are sensitive to a limited range of frequencies around a central frequency $\nu_0$. 
The radio flux at a given frequency can be evaluated by considering the spectral shape of the signal.
Radio pulsars are usually characterized by a power-law spectral shape \citep[see][]{Jankowski2018}. 
Therefore to compute the flux density at a given frequency $\nu$ we can use the following relation:
%--------------------------------------------------------------
\begin{align}
    S_{\nu}(\nu) = S_{\nu, 0} \left( \frac{\nu}{\nu_0} \right)^{\alpha} = \frac{S (\alpha + 1)}{\nu_{\rm max}^{\alpha+1} - \nu_{\rm min}^{\alpha+1}} \nu^{\alpha},  
\end{align}
%--------------------------------------------------------------
where we used the fact that $S$ is the flux integrated over the entire frequency range between $\nu_{\rm min}$ and $\nu_{\rm max}$:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_integral_flux}
    S = \int_{\nu_{\rm min}}^{\nu_{\rm max}} S_{\nu}(\nu) {\rm d} \nu = S_{\nu,0} \frac{\nu_0^{-\alpha}}{\alpha + 1} \left( \nu_{\rm max}^{\alpha+1} - \nu_{\rm min}^{\alpha+1} \right).
\end{align}
%--------------------------------------------------------------

We can also define the fluence of this signal by integrating the flux over the interval of time defined by the spin period:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_fluence}
    \mathcal{F}_{\nu}(\nu)  & = \int_{0}^{P} S_{\nu}(\nu, t) {\rm d} t = S_{\nu}(\nu)w,
\end{align}
%--------------------------------------------------------------
where for simplicity we considered a rectangular top-hat pulse shape with intrinsic width $w$.
The fluence has units of [erg cm$^{-2}$] and is a measure of the total energy carried by a radiation pulse passing through a unit surface area.

However, to reach the Earth the signal has to propagate through the interstellar medium which is characterized by clumpy regions with different densities where gas can be completely ionized.
In the presence of ionized gas, the electromagnetic interaction between the photons and the free electrons causes a delay in the propagation of the light, which is a function of photon frequency. More energetic photons tend to push past the free electrons with little effect on their propagation speed, whereas lower frequency photons (like radio waves) are more significantly delayed. 
We quantify these effects by introducing the refraction index $n$, which for a non-magnetized, non-relativistic and ionized plasma is given by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_refraction_index}
    n(\nu) & = \sqrt{ 1 - \left( \frac{\nu_{\rm p}}{\nu} \right)^2},
\end{align}
%--------------------------------------------------------------
where $\nu_{\rm p}$ is the so-called plasma frequency for a non-magnetized plasma:
%--------------------------------------------------------------
\begin{align}
    \nu_{\rm p} = \left( \frac{e^2 n_e}{\pi m_e} \right)^{1/2} \simeq \unit[8.98]{kHz} \left( \frac{n_e}{\unit[1]{cm^{-3}}} \right)^{1/2}. 
\end{align}
%--------------------------------------------------------------
The delay in the arrival time of a wave of frequency $\nu$ with respect to the arrival time in vacuum can be estimated to be \citep[see][]{Lorimer2012}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_delay_DM}
    \delta t(\nu) & = \left( \int_0^d \frac{{\rm d}l}{n(\nu) c} \right) - \frac{d}{c} \simeq \int_0^d \frac{{\rm d} l}{c} \frac{\nu_{\rm p}^2}{2 \nu^2} \nonumber \\ 
                  & = \frac{e^2}{2 \pi m_e c} \nu^{-2} \int_0^d {\rm d} l n_e(l) \nonumber \\ 
                  & \simeq \unit[0.41]{s} \left( \frac{\nu}{\unit[1]{GHz}} \right)^{-2} \frac{DM}{\unit[100]{pc \, cm^{-3}}},
\end{align}
%--------------------------------------------------------------
where we assumed $\nu_{\rm p} \ll \nu$. 
The integral is performed along the line of sight $l$, over a distance $d$. The electron column density along the line of sight defines the dispersion measure $DM$.
Therefore to recover the original pulse shape, the detected signal has to be de-dispersed by re-aligning the observations of delayed pulses at different frequencies.
However, a radio detector has a finite frequency resolution. Usually, the total bandwidth of the instrument is divided into different channels, each one sensitive to photons in a particular range of frequencies $\Delta \nu_{\rm ch}$.
Since photons collected by a given spectral channel cannot be distinguished in frequency, the de-dispersion cannot be applied per channel. To obtain an estimate of the residual intra–channel dispersion smearing contribution to the observed pulse width we instead differentiate Equation~\eqref{eq:ch2_delay_DM} with respect to the frequency $\nu$ to find the amount of delay per unit frequency interval and multiply by the minimum frequency bin $\Delta \nu_{\rm ch}$ of the instrument:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_smearing_DM}
    \Delta t_{DM} & = \left| \frac{{\rm d} \delta t}{{\rm d} \nu} \right| \Delta \nu_{\rm ch}  \nonumber \\ 
                  & = \frac{e^2}{\pi m_e c} \nu^{-3} \Delta \nu_{\rm ch} DM \nonumber \\ 
                  & \simeq \unit[0.83]{ms} \left( \frac{\nu}{\unit[1]{GHz}} \right)^{-3} \frac{\Delta \nu_{\rm ch}}{\unit[1]{MHz}} \frac{DM}{\unit[100]{pc \, cm^{-3}}}.
\end{align}
%--------------------------------------------------------------

Furthermore, the electron density in the medium is not homogeneous and shows variations over a wide range of length scales. The distribution of scales of these variations is affected by the presence of turbulence in the medium, which introduces a relative motion between the source, the inhomogeneous
clumps and the observer. As the electromagnetic signal propagates, it encounters several such irregularities depending on the travelled distance $d$. At each encounter, it is delayed and deflected in a frequency-dependent way. The result is that a sharp pulse emitted by a point source is detected as a scattered-broadened pulse whose intensity decays exponentially with a characteristic time $\tau_{\rm sc}$ which depends on the signal
frequency and distance of the source \citep[see][]{Lorimer2012}. By assuming a Kolmogorov turbulence power spectrum for the inhomogeneity length scales \citep{Kolmogorov1941} the broadening timescale due to scattering is given by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_scattering_timescale}
    \tau_{\rm sc} & \propto d^{2.2} \nu^{-4.4}.
\end{align}
%--------------------------------------------------------------
Some studies show evidence of a relation between the scattering broadening timescale and the dispersion measure. For example, by using a sample of scattering measurements from 124 pulsars detected at $\unit[327]{MHz}$ by the Ooty Radio Telescope in Southern India, \cite{Krishnakumar2015} found the following empirical relation:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_tausc_DM_relation}
    \tau_{\rm sc} = \unit[3.6 \times 10^{-9}]{s} \left(\frac{DM}{\unit[1]{pc \, cm^{-3}}} \right)^{2.2} \left[ 1.0 + 1.94 \times 10^{-3} \left(\frac{DM}{\unit[1]{pc \, cm^{-3}}} \right)^{2.0} \right].
\end{align}
%--------------------------------------------------------------
This empirical relation is useful to estimate the scattering timescale for sources which only have a measurement of the dispersion measure. 

Additionally, there are instrumental effects that contributes to the broadening of the pulse shape during the digital processing of the radio signal. The most relevant effect is given by the detector sampling time which limits the time resolution of the pulse and introduce an uncertainty in the pulse duration given by $\Delta t_{\rm samp}$.

As a result of the effects discussed here, the observed duration $w_{\rm obs}$ of a radio pulse is larger than the intrinsic duration $w$ and is given by the quadratic sum of the contributions described above as reported in \cite{Cordes2003}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_eff_pulse_width}
    w_{\rm obs} \simeq \sqrt {w^2 + \Delta t_{DM}^2 + \tau_{\rm sc}^2 + \Delta t_{\rm samp}^2},
\end{align}
%--------------------------------------------------------------

As the pulse propagates, gets dispersed and broadens, its fluence is defined by Equation~\eqref{eq:ch2_fluence} is conserved. Therefore the flux of the pulse detected on Earth can be found by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_obs_radio_flux}
    S_{\nu}(\nu) w  & = S_{\nu,\rm obs}(\nu) w_{\rm obs} \, \Longrightarrow \, S_{\nu,\rm obs}(\nu) = \frac{S_{\nu}(\nu) w}{w_{\rm obs}}.
\end{align}
%--------------------------------------------------------------

\subsection{Pulsar pseudo-luminosity} \label{sec:ch2_pseudo_luminosity}

By inverting the steps described in the last section, one should in principle be able to estimate the intrinsic luminosity of a pulsar from the observed quantities.
Usually in pulsar radio surveys the flux $S_{\nu, \rm mean}$ averaged over a period and at the observation frequency $\nu_0$ is reported. Assuming for simplicity a rectangular pulse shape with peak flux $S_{\nu, \rm obs}$ and observed width $w_{\rm obs}$ this is given by:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_mean_radio_flux}
    S_{\nu, \rm mean}(\nu_0) & = \frac{\int_0^P S_{\nu, \rm obs}(\nu_0, t) {\rm d}t}{P} = \frac{S_{\nu, \rm obs}(\nu_0) w_{\rm obs}}{P}.
\end{align}
%--------------------------------------------------------------
To recover the intrinsic flux $S(\nu_0)$ we need to find the intrinsic pulse width. From Equation~\eqref{eq:ch2_eff_pulse_width} we have:
%--------------------------------------------------------------
\begin{align}
    w \simeq \sqrt {w_{\rm obs}^2 - \Delta t_{DM}^2 - \tau_{\rm sc}^2 - \Delta t_{\rm samp}^2}.
\end{align}
%--------------------------------------------------------------
By combining Equation~\eqref{eq:ch2_obs_radio_flux} and Equation~\eqref{eq:ch2_mean_radio_flux} with the previous equation we then find:
%--------------------------------------------------------------
\begin{align} 
    S_{\nu}(\nu_0) & \simeq S_{\nu, \rm mean}(\nu_0) \frac{P}{\sqrt {w_{\rm obs}^2 - \Delta t_{DM}^2 - \tau_{\rm sc}^2 - \Delta t_{\rm samp}^2}} = \frac{S_{\nu, \rm mean}(\nu_0)}{\delta},
\end{align}
%--------------------------------------------------------------
where here we define the intrinsic duty cycle $\delta \equiv w/P$.
Finally using Equation~\eqref{eq:ch2_radio_flux} and Equation~\eqref{eq:ch2_solid_angle} we obtain for the intrinsic luminosity density:
%--------------------------------------------------------------
\begin{align} 
    L_{\nu}(\nu_0) \simeq \frac{8 \pi}{\delta} \sin^2\left( \frac{\rho_{\rm em}}{2} \right) d^2 S_{\nu, \rm mean}(\nu_0).
\end{align}
%--------------------------------------------------------------
And integrating over the frequencies (Equation~\eqref{eq:ch2_integral_flux}) we obtain the bolometric intrinsic radio  luminosity:
%--------------------------------------------------------------
\begin{align} 
    L \simeq \frac{8 \pi}{\delta} \sin^2\left( \frac{\rho_{\rm em}}{2} \right) d^2 S_{\rm mean}(\nu_0) \frac{\nu_0^{-\alpha}}{\alpha + 1} \left( \nu_{\rm max}^{\alpha+1} - \nu_{\rm min}^{\alpha+1} \right).
\end{align}
%--------------------------------------------------------------

However, a precise estimate of the intrinsic radio luminosity is not trivial for the following reasons:
\begin{itemize}
    \item In most cases estimating the angular aperture $\rho_{\rm em}$ of the radio beam and the intrinsic pulse width $w$ can be challenging. Pulsars often exhibit intricate emission patterns, making it highly complicated to deduce the emission geometry and accurately determine the pulse width. One possibility to estimate the beam angular aperture from the spin period is to use the relation given by Equation~\eqref{eq:ch2_beam_angular_aperture}, which has been confirmed by observation despite some uncertainties \citep{Rankin1993, Maciesiak2012}. Additionally, removing the broadening effects described above from the observed pulse width $w_{\rm obs}$ is not a straightforward task, as it can be difficult to differentiate these effects from the inherent properties of the pulse shape \textbf{REF?}.

    \item Accurate modelling of radio pulsar spectra is not always possible. Radio spectra appear to be different for every pulsar. As shown in \cite{Jankowski2018} in many cases a single power-law model describes the observed spectrum well but many pulsars deviate from this simple behaviour. 

    \item The estimate of the distance $d$ is subject to many uncertainties. For radio pulsars, the main way to estimate the distance relies on models for the electron density distribution in the Galaxy. Three main models have been developed over the years from \citep[see][]{Taylor1993, Cordes2002, Yao2017}. By knowing the $DM$ value and the sky position of the pulsar, these models predict the amount of free electrons along the line of sight and give a rough estimate of the distance. However, due to the complexity of modelling the Galactic structures, these models suffer from a lot of uncertainties. The relative error on the distance estimated from the $DM$ values could indeed be around 40 \% \citep{Yao2017}. 
\end{itemize}

Due to these uncertainties fiducial values are usually adopted for the unknown quantities \citep[see][]{Lorimer2012}. For example by considering a fixed beam aperture of $\rho_{\rm em} \sim \unit[6]{deg}$, the ratio between the intrinsic pulse width and the spin period (the duty cycle) of $\delta = 0.04$,  a radio frequency range from $\nu_{\rm min} = \unit[10]{MHz}$ to $\nu_{\rm max} = \unit[100]{GHz}$ \citep[see for example][]{Izvekova1981, Morris1997}, and a spectral index $\alpha = -1.6$ \citep{Jankowski2018}, we have a pseudo luminosity of:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_pseudo-luminosity}
    L_{\nu, \rm pseudo}(\unit[1.4]{GHz}) & \simeq \unit[7.4 \times 10^{27}]{erg \, s^{-1}} \left( \frac{S_{\nu, \rm mean}(\unit[1.4]{GHz})}{\unit[1]{mJy}} \right) \left( \frac{d}{\unit[1]{kpc}} \right)^2.
\end{align}
%--------------------------------------------------------------
However note that performing a population study and applying this expression to different pulsars without taking into account differences in their intrinsic duty cycles and beam geometries will mask eventual intrinsic correlations between the intrinsic luminosity and the spin-down properties like $P$, $\dot{P}$ and $\dot{E}_{\rm rot}$. This is because $\rho_{\rm em}$ and $w$ have a non-trivial dependence on the spin period (see Section~\ref{sec:ch2_radio_em_geometry}). For example \cite{Posselt2023} recently showed that the radio pseudo-luminosity has a shallow dependence on the spin-down energy loss $L_{\nu, \rm pseudo} \propto \dot{E}_{\rm rot}^{0.15}$ \citep[see also][]{Szary2014}. However, this might not be a proof of the absence of intrinsic correlations between the intrinsic radio luminosity and the rotational properties. 


\subsection{Radiometer equation}

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Haslam_sky_temperature.pdf}
\caption[Sky temperature distribution]{Sky temperature distribution at 408 MHz from \cite{Haslam1982}, refined by \cite{Remazeilles2015} \citep[Figure taken from][]{Remazeilles2015}.}
\label{fig:ch2_T_sky_distribution}
\end{figure*}
%----------------------------------------------------

In this section we will describe how we can model the sensitivity of a radio telescope which is a crucial aspect to determine which pulsars are detectable. We follow \cite{Lorimer2012}.

Consider the observation of a signal with peak flux density $S_{\nu,\rm obs}(\nu)$ (in $\unit[]{erg \, s^{-1} \, Hz^{-1}}$), performed with an antenna telescope of effective area $A_{\rm eff}$. 
We consider an unpolarized signal where the electric field vector changes randomly in all possible directions perpendicular to the direction of wave propagation.
Since each of the two orthogonal polarization directions contributes half the total flux, the power received from the source per unit frequency bandwidth and polarization is $P_{\rm source} = S_{\nu, \rm obs}(\nu) A_{\rm eff} / 2$. Now consider modelling the antenna as a simple circuit consisting of a resistive load at temperature $T$. The thermal motions of the electrons inside the resistor induce a time variable voltage in this circuit which produces a power per unit frequency bandwidth that can be translated into a temperature by $P_{\rm circuit} = k_{\rm B} T$, where $k_{\rm B}$ is the Boltzmann constant \citep{Nyquist1928}. Therefore an incident electromagnetic wave with a power per unit frequency $P_{\rm source}$ will produce a power in the circuit given by $P_{\rm circuit} = P_{\rm source}$. It follows that:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_flux_antenna_eq}
    S_{\nu, \rm obs}(\nu) & = \frac{2 k_{\rm B} T_{\rm source}}{A_{\rm eff}} = \frac{T_{\rm source}}{G},
\end{align}
%--------------------------------------------------------------
where we define the antenna gain as $G \equiv A_{\rm eff} / ( 2 k_{\rm B} )$ which is a measure of the antenna sensitivity. In other words the source of flux density $S_{\nu, \rm obs}( \nu )$ have an equivalent temperature $T_{\rm source}$ given by Equation~\eqref{eq:ch2_flux_antenna_eq} in the telescope system.

However real observing systems have many sources of noise, that can be
modelled as a background system temperature $T_{\rm sys}$. The system temperature accounts for the noise contributions from the receiver, transmission lines, and other components of the radio telescope system which are represented as a receiver temperature $T_{\rm rec}$. Furthermore, $T_{\rm sys}$ includes any spurious background signals coming from the sky with an equivalent temperature $T_{\rm sky}(l, b)$ which is a function of galactic sky coordinates $(l, b)$.
Figure~\ref{fig:ch2_T_sky_distribution} shows the Sky temperature distribution measured at $\unit[408]{MHz}$ as a function of equatorial coordinates \citep{Haslam1982, Remazeilles2015}. This temperature can be re-scaled to the central frequency of the survey assuming a frequency spectrum $T_{\rm sky} \propto \nu^{-2.6}$ \citep{Lawson1987, Johnston1992}.
Therefore in general we can write $T_{\rm sys} = T_{\rm rec} + T_{\rm sky}(l, b)$. These noise sources are usually much larger than the faint signals we receive from astronomical sources. For this reason, to establish if a source is detectable we rely on the concept of signal to noise ratio which measures deviations from the random noise oscillation of the receiver.   

The root mean square fluctuations $\sigma_T$ of the noise in the telescope for a given generic temperature $T$ decreases with the square root of the number of measured polarizations $n_{\rm p}$, the receiver frequency bandwidth $\Delta \nu_{\rm bw}$ and integration time $t_{\rm int}$ \citep{Dicke1946}:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_T_fluctuations}
    \sigma_{T} & = \frac{T}{\sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}}.
\end{align}
%--------------------------------------------------------------
This equation is known as the radiometer equation and is used to perform estimation of the system sensitivity.

Consider an observation of a pulsar for a total integration time $t_{\rm int}$. The pulsar has a top-hat pulse shape with width $w_{\rm obs}$, periodicity $P$ and an associated temperature $T_{\rm source}$. Over the whole integration time, the pulsar is on over a time $t_{\rm on} = t_{\rm int} w_{\rm obs} / P$ and it is off for a time $t_{\rm off} = t_{\rm int} (P - w_{\rm obs}) / P$.
For the pulsar to be detectable, its signal has to exceed the noise fluctuations in the system during the integration time. The ratio between $T_{\rm source}$ and the system noise fluctuations $\sigma_{T_{\rm sys}}$ define the signal to noise ratios $S/N$. To have a significative detection the $S/N$ has to surpass a threshold that is usually taken to be above 5 \citep[see][]{Vivekanand1982, Lorimer2012}. The root mean square noise fluctuations during the integration time can be computed as the quadrature sum:
%--------------------------------------------------------------
\begin{align} 
    \sigma_{T_{\rm sys}} & = \sqrt{ \sigma_{T_{\rm on}}^2 + \sigma_{T_{\rm off}}^2} \nonumber \\
            & = \sqrt{ \left( \frac{T_{\rm source} + T_{\rm sys}}{\sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm on}}} \right)^2  + \left( \frac{T_{\rm sys}}{\sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm off}}} \right)^2} \nonumber \\
            & \simeq \frac{T_{\rm sys}}{\sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}} \frac{P}{\sqrt{w_{\rm obs} (P - w_{\rm obs})}},
\end{align}
%--------------------------------------------------------------
where we used Equation~\eqref{eq:ch2_T_fluctuations} and made the approximation that $T_{\rm source} \ll T_{\rm sys}$.
We can therefore define the signal-to-noise ratio as:
%--------------------------------------------------------------
\begin{align}
    S/N &\equiv \frac{T_{\rm source}}{\sigma_{T_{\rm sys}}} = \frac{T_{\rm source} \sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}}{T_{\rm sys}} \frac{\sqrt{w_{\rm obs} (P - w_{\rm obs})}}{P} \nonumber \\
    &= \frac{S_{\rm obs}(\nu) \sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}}{G T_{\rm sys}} \frac{\sqrt{w_{\rm obs} (P - w_{\rm obs})}}{P},
\end{align}
%--------------------------------------------------------------
where in the last step we used Equation~\eqref{eq:ch2_flux_antenna_eq}.
To take into account system imperfections, for example due to the digitization of the signal, a degradation factor $\beta \sim 1.5$ is commonly introduced so that the previous equation becomes: 
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_StoN_radiometer_eq}
    S/N = \frac{S_{\nu, \rm obs}(\nu) \sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}}{\beta G T_{\rm sys}} \frac{\sqrt{w_{\rm obs} (P - w_{\rm obs})}}{P}.
\end{align}
%--------------------------------------------------------------
If we consider the period-averaged flux by substituting Equation~\eqref{eq:ch2_mean_radio_flux} into \eqref{eq:ch2_StoN_radiometer_eq} we find:
%--------------------------------------------------------------
\begin{align} \label{eq:ch2_StoN_radiometer_eq_Smean}
    S/N = \frac{S_{\nu, \rm mean}(\nu) \sqrt{n_{\rm p} \Delta \nu_{\rm bw} t_{\rm int}}}{\beta G T_{\rm sys}} \sqrt{ \frac{P - w_{\rm obs}}{w_{\rm obs}}}.
\end{align}
%--------------------------------------------------------------
This equation shows that the narrower the pulse, the bigger the signal-to-noise ratio, hence the easier it is to detect the pulsar.

We now have all the ingredients in place to study the properties of radio pulsars.
Before looking at this in detail, we however first turn our attention to machine learning, introducing the key concepts crucial for the following chapters.

%--------------------------------------------------------------------------------------------   

==> Chapters/Chapter_intro_NS.tex <==
\chapter{Neutron stars, an introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Introduction}

The existence of neutron stars was first proposed in 1934, two years after the discovery of the neutron itself \citep{Chadwick1932}, when \cite{Baade1934} wondered if a celestial body made entirely of neutrons might remain after a supernova explosion. 
It was not until the 1960s that Baade and Zwicky’s hypothetical neutron stars were finally detected. While working as a PhD student at the University of Cambridge Jocelyn Bell Burnell noticed a strange, regularly pulsed radio signal in the data collected using the Mullard Radio Astronomy Observatory. These signals were initially interpreted as the result of radial pulsations in either a white dwarf or a neutron star \citep{Hewish1968}.
This groundbreaking discovery opened up new avenues for exploring the intriguing relationship between neutron stars and their potential to emit highly focused beams of electromagnetic radiation. Soon after it was suggested by \cite{Pacini1968} and \cite{Gold1968} that coherent emission could occur in rotating neutron stars with strong magnetic fields where particles could be accelerated up to relativistic speeds and emit beams of electromagnetic radiation. This can be detected as pulsed signals as the neutron star rotates like a lighthouse. Hence the name "pulsar" was coined.
By that time about 20 similar objects had been identified including a source in the Crab nebula \citep{Staelin1968, Comella1969} and one in the Vela supernova remnant \citep{Large1968}. The identification of these pulsars with rotating neutron stars was in the end confirmed by the measurement of a spin-down in the period of the Crab pulsar \citep{Richards1969} as a spin-down is more easily achieved in rotating objects rather than in pulsating ones. Furthermore, the identification of some pulsars with supernova remnants further supported the initial idea of Baade and Zwicky.

With subsequent technological advancements in observational astronomy, the population of known neutron stars has grown exponentially. Since the first detection, around 3000 pulsars have been discovered, not only in the radio band \citep{Manchester2005}\footnote{see the ATNF pulsar catalog \url{https://www.atnf.csiro.au/research/pulsar/psrcat/}}. Pulsars can be radio-quiet or emit across a wider wavelength range from radio to gamma-rays. However, an enduring challenge lies in accurately characterizing their birth properties as well as deciphering the mechanisms that regulate their formation and evolution. Untangling the contributing factors, such as the initial magnetic field strength and spin period distributions, holds paramount importance in understanding the diverse outcomes of stellar evolution and the underlying physical processes within core-collapse supernovae. By combining observational constraints with data analysis and sophisticated numerical simulations, researchers can refine existing theoretical models and shed light on the complex physical processes involved in the formation and evolution of these dense remnants.

In this chapter we summarize the main properties of neutron stars and the challenges to model their Galactic population.  

%----------------------------------------------------------------------------------------

\section{Formation} 

The progenitors of neutron stars are massive stars of spectral types O and B, characterized by initial masses between around 8 and 25 \msun \citep{Shapiro1983}. 
In general, depending on its initial mass, a star spend from a few million years up to more than ten billion years on the main sequence, burning hydrogen into helium \citep{Phillips1994, Prialnik2000}. In this stage, the thermal pressure released by the thermonuclear fusion reactions in its core supports the star against gravitational collapse. However, the more massive a star is, the faster it consumes its nuclear fuel and the faster it evolves towards its death. After exhausting all the hydrogen in the core the thermal pressure support coming from hydrogen burning vanishes. The inner regions of the star, now mainly composed of helium "ashes", start to contract due to their own gravity. As a consequence they heat up while the outer envelope expands and cools down. The star becomes a red giant. As the temperature in the helium core grows upon contraction, new nuclear fusion reactions are triggered. Helium starts to burn and to be converted into carbon, oxygen and neon. The released energy allows to restore again the equilibrium with gravity and the star enters a new stable phase that usually lasts one-tenth of the main sequence phase. However, once the helium fuel is exhausted, the core (now composed mainly of oxygen and carbon) starts to contract again. 

In stars with an initial mass of less than about 8 \msun, the dense core reaches equilibrium in a new state of matter called a degenerate electron gas. In this state, the stellar core is supported against further gravitational contraction thanks to the pressure exerted by the electrons due to the Pauli exclusion principle, even in the absence of nuclear reactions. In the meanwhile, the outer envelopes of the star expand further and are gradually dispersed. What is left is the exposed core of the star with a mass of $\sim 0.5 - 1$ \msun and a radius of $\sim \unit[10^8]{cm}$, made primarily by helium, carbon and oxygen. A white dwarf has formed.

For stars with an initial mass greater than about 8 \msun the electron degeneracy pressure is not enough to counteract gravity. Therefore they continue the sequence of core contraction and ignition of new nuclear reactions. As time goes by the inner core reaches temperatures and densities favourable for the synthesis of progressively heavier elements. After hydrogen and helium, these massive stars burn carbon, neon, oxygen, and silicon on progressively faster timescales. In this way, they undergo all the stages of nuclear burning up to the production of elements in the "iron group" with atomic number $A = 56$. The iron group elements are the most tightly bound nuclei and their synthesis into heavier elements consumes, rather than releases, energy. Since no further energy can be released from the nuclear fusion reactions as the iron core grows it becomes unstable and is not further supported against gravitational collapse.
As the iron core approaches the Chandrasekhar mass limit of about $1.4$ \msun \citep{Chandrasekhar1931}, the central temperature and density reaches values of about $\sim \unit[10^9]{K}$ and $\sim \unit[10^9]{g \, cm^{-3}}$ respectively. The temperature is high enough that nuclear photo-disintegration is triggered: the abundant energetic photons trapped in the hot dense core are partly consumed to unbind nuclei into lighter elements in endothermic reactions. In such a way the photon radiation pressure is lost. 
Furthermore, at such densities, reactions like electron capture $e^- + p \longrightarrow n + \nu_e$ become energetically favourable. The electrons are absorbed by the nuclei which become very neutron-rich in what is called neutronization. This process depletes the core of electrons and their supporting degeneracy pressure. Futhermore a big amount of energy is carried away by neutrinos. This leads to an almost unrestrained collapse of the stellar core on a free-fall timescale of a few seconds. 

As the collapse proceeds, the core central density increases to the point that neutrons start to drip out of the nuclei and form a degenerate gas. At densities $\gtrsim \unit[10^{14}]{g \, cm^{-3}}$, the nuclei are completely dissolved into homogeneous nuclear matter mostly composed of neutrons. If the mass of the collapsing core is not too high ($\lesssim 3$ \msun), the degeneracy pressure exerted by the neutrons is ﬁnally able to halt the collapse. This triggers a shock wave, that propagates outwards through the collapsing stellar layers and blows them up in what is observed as a supernova explosion.
What is left is a very hot and compact remnant of mass $M \sim 1 - 2$ \msun and radius $R \sim \unit[10^6]{cm}$: a neutron star.

%---------------------------------------------------------------------------------------

\section{Internal structure and the mass-radius relation} \label{sec:ch1_internal_structure_MR_relation}

%----------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{M_R_relation.pdf}
\caption[Neutron star mass-radius relation.]{Neutron star mass-radius curves corresponding to different equations of state calculated under different physical assumptions and using a range of computational approaches \citep[see][for more details]{Ozel2016} \citep[Figure taken from][]{Ozel2016}.}
\label{fig:ch1_mass_radius}
\end{figure*}
%----------------------------------------------------

To our knowledge, neutron stars are the most compact objects in the Universe where matter can still reach a stable configuration under the effect of extreme gravity. Their compactness, deﬁned by the ratio between their Schwarzschild radius $R_{\rm S} = \frac{2GM_{\rm NS}}{c^2}$ and their radius $R_{\rm NS}$, is of the order:
%--------------------------------------------------------------------
\begin{align}
    \frac{R_{\rm S}}{R_{\rm NS}} \simeq 0.376 \left( \frac{M_{\rm NS}}{1.4 M_{\odot}} \right) \left( \frac{R_{\rm NS}}{\unit[11]{km}} \right)^{-1}.
\end{align}
%--------------------------------------------------------------------
This is close to the most extreme value given by a Schwarzschild black hole where the compactness is 1. 
The density grows from values less than $\unit[10^4]{g \, cm^{-3}}$ in the outermost envelope to nuclear density values $\unit[10^{14} - 10^{15}]{g \, cm^{-3}}$ in the neutron star core. As you move radially into the star from the surface, the pressure increases to support the increasing weight of the material above any given point. Hence the structure and state of matter change as we move inside \citep[see][for a review]{Chamel2008}. 
The outer layers ($\sim \unit[100]{m}$) are a liquid ocean of heavy nuclei of the iron group and degenerate free electrons. As one moves into the crust ($\sim \unit[1]{km}$), the nuclei are more packed together and the Coulomb interactions between them begin to dominate over the thermal energy. The nuclei rearrange themselves to form a solid elastic lattice. On the other end, the degenerate free electrons become relativistic.  
At the basis of the crust and the interface with the core, the heavy nuclei become more and more neutron-rich and deformed into cylindrical and planar shapes. This is the so-called "nuclear pasta phase".
Moving into the inner core the nuclei are completely dissolved into an ocean of free neutrons togeteher with protons, ultra-relativistic electrons and muons. The neutron degenerate pressure supports the neutron star against collapse. However, at these extreme densities, the exact composition and the properties of matter in the inner core are not clear as exotic particles may be present. Therefore the exact equation of state, i.e. the relation linking pressure and density, for neutron stars is still unknown. 
\citet{Oppenheimer1939, Tolman1939}  were the first ones to propose an equation of state of a relativistic gas of degenerate neutrons and a model for the hydrostatic equilibrium of general relativistic bodies also known as Oppenheimer-Volkoff-Tolmann equation:
%--------------------------------------------------------------------
\begin{align}
    \frac{{\rm d}p(r)}{{\rm d}r} = \frac{G M(r) \rho(r)}{r^2} \left[ 1 + \frac{p(r)}{\rho(r) c^2} \right] \left[ 1 + \frac{4\pi r^3 p(r)}{ M(r) c^2} \right] \left[1 - \frac{2GM(r)}{c^2 r} \right]^{-1},
\end{align}
%--------------------------------------------------------------------
where $p(r)$ and $\rho(r)$ are the pressure and density, respectively, and $M(r)$ is the mass within the radius $r$.
In particular, the solution of this equation maps a given equation of state to the corresponding mass-radius relation, linking in this way the microscopic to the macroscopic properties of the star. Since then the knowledge of the behaviour of matter at nuclear densities has progressed and several models for the equation of state of neutron stars have been proposed. 
The uncertainty is still big. For a given mass, these equations of state allow a range of radii between $\sim \unit[7]{km}$ up to $\sim \unit[16]{km}$ (see Figure~\ref{fig:ch1_mass_radius}).
Therefore, to constrain the equation of state for the neutron star matter, it is crucial to obtain independent measurements of the mass and radius \citep[see][for a review]{Ozel2016}.   

The currently available measurements of neutron star masses come primarily from the study of neutron stars in binary systems. Up to now the minimum mass estimated for a neutron star is $1.174 \pm 0.004$ \msun for PSR J0453+1559 \citep{Martinez2015} while the heaviest neutron star is PSR J0952--0607 which has an estimated mass of $2.35 \pm 0.17$ \msun \citep{Romani2022}. Finding the maximum mass for neutron stars is of particular relevance since it can rule out the equations of state that predict maximum masses below this value. 

Until recently, the measurement of neutron-star radii mainly relied on X-ray observations and spectral analysis of quiescent and accreting neutron stars \citep{Miller2019, Riley2019}. The typical estimates for the radii obtained with these methods are in the range $\unit[10 - 14]{km}$ \citep[see, e.g.,][]{Steiner2018}. However, these analyses are often affected by systematics that are difficult to quantify. After the serendipitous detection of the famous binary neutron-star merger GW170817 and its electromagnetic counterparts \citep{Abbott2017a, Abbott2017b, Abbott2017c}, the beginning of the multi-messenger observation era has opened a new window on this front. For example, by combining electromagnetic and gravitational wave data \cite{Margalit2017} managed to put constraints on the maximum neutron star mass. \citet{Capano2020, Raaijmakers2021} combined nuclear theory with the data from the gravitational waves and electromagnetic emission from this event using a Bayesian framework. They were able to constrain the radius of a neutron star with mass $M = 1.4$ \msun to values around $\unit[11 - 12]{km}$.

%--------------------------------------------------------------------------------------------

\section{Spin periods} \label{sec:ch1_spin_periods}

By identifying the periodicity of the arrival time of pulses of radiation with the neutron star spin periods implies that these celestial bodies rotate at very high speeds. From the observed population their spin periods range from a few milliseconds to a few tens of seconds (see Figure~\ref{fig:ch1_PPdot_diagram}). The majority of these measurements come from radio timing analysis which has also unveiled that their spin periods increase with time at rates between around $\unit[10^{-20}]{s \, s^{-1}}$ and $\unit[10^{-10}]{s \, s^{-1}}$. This suggests that generally neutron stars spin down over time and they should be born with even shorter rotation periods.

Several works involving analyses of young supernova remnants \citep[e.g.][]{Chevalier2005}, population synthesis studies \citep[e.g.][]{Popov2012, Faucher2006, Gullon2014} and supernova simulations \citep[e.g.][]{Ott2006, Janka2021}, have suggested that the birth spin periods of neutron stars should range between a few tens of milliseconds up to a few hundreds of milliseconds. However, the origin of such fast rotation is still unclear.

A first insight into how neutron stars could achieve these fast rotation can be gained by considering the angular momentum conservation during the collapse of the iron core. For an order of magnitude estimation we consider a core with mass $M_{\rm core} \sim 1.4$ \msun, radius comparable to our Sun $R_{\rm core} \sim \unit[10^{11}]{cm}$ and spin period $P \sim \unit[1]{day}$. From the conservation of angular momentum, we get that:
%------------------------------------------------------------------------
\begin{align}
    M_{\rm core} R_{\rm core}^2 \omega_{\rm core} \sim  M_{\rm NS} R_{\rm NS}^2 \omega_{\rm NS},
\end{align}
%------------------------------------------------------------------------
where $\omega = 2 \pi / P$ is the spin angular velocity and we assumed mass conservation during the core collapse, i.e., $M_{\rm core} \sim  M_{\rm NS}$. During the collapse, as the radius shrinks to $R_{\rm NS} \sim \unit[10^{6}]{cm}$ reducing the moment of inertia by a factor $\sim 10^{10}$, the angular velocity should increase by the same amount. As a consequence, newborn neutron stars should spin with periods of the order of milliseconds.

However angular momentum conservation is not the only ingredient to explain the neutron star's fast rotation. Various mechanisms acting during and after the supernova explosion could contribute to spinning up or spinning down the collapsing core and the newly formed neutron star. During the core collapse and the development of the supernova, hydrodynamical instabilities and turbulent motion of mass could cause asymmetric mass ejection in the supernova. This asymmetry imparts accelerating forces on the core over timescales from several seconds to hours. In this way, the newly formed neutron star is displaced from the centre of the collapse and receives a kick that can be of several hundreds of kilometers per second \citep[see, e.g., ][but also Chapter~\ref{Chapter6}]{Hobbs2005}. As the neutron star moves in the supernova ejecta it can accrete a fraction of the matter that has remained gravitationally bound. This anisotropic accretion of mass could transfer a relevant amount of angular momentum to the compact remnant after the development of the supernova \citet{Janka2021, Coleman2022}. This scenario suggests also a possible link between the origin of the fast neutron stars' proper motion and their spin period.

%--------------------------------------------------------------------------------------------

\section{Magnetic fields} \label{sec:ch1_magnetic_field}

To our knowledge neutron stars are also the strongest magnets in the Universe. A direct measurement of the magnetic field strength is not straightforward though. One possibility is through the detection of cyclotron lines, that generally appear as absorption features in the high-energy X-ray spectra of systems containing highly magnetized neutron stars. Almost all the observations of cyclotron absorption features come from neutron stars accreting matter from a stellar companion, also called X-ray binary pulsars. These features are produced as the photons produced by the hot column of plasma accreted onto the neutron star's magnetic poles are resonantly scattered by charged particles gyrating around the magnetic field lines \citep[see for example][for a review]{Staubert2019} \textbf{REF?}. 

However, generally, neutron star magnetic fields are indirectly estimated from their rotational properties. 
The commonly adopted explanation for this rotational energy loss is that the neutron star experiences an electromagnetic torque generated by a very powerful dipolar magnetic field (see Section~\ref{sec:ch2_dip_spindown_evol}).
With this assumption, from the measurements of the spin period and spin period derivative one can infer dipolar magnetic field values that range between $\unit[10^8]{G}$ to almost $\unit[10^{15}]{G}$.

How such strong magnetic fields are generated is still a matter of debate.
One idea is that the neutron star inherits the magnetic field of the parent OB star. In this fossil field hypothesis, during the core collapse the magnetic field gets amplified due to magnetic flux freezing \citep{Ferrario2006, Hu2009}. 
Ordinary OB stars have a magnetic field of the order of $B \sim \unit[10^2]{G}$ with some of them exceeding $\unit[10^3]{G}$. 
% See: https://ui.adsabs.harvard.edu/abs/2014A%26A...564L..10H/abstract
From the conservation of the magnetic flux, we have that:
%------------------------------------------------------------------------
\begin{align}
    B_{\rm core} R_{\rm core}^2 \sim  B_{\rm NS} R_{\rm NS}^2.
\end{align}
%------------------------------------------------------------------------
As the core radius contracts by a factor $\sim 10^5$, the magnetic field should be amplified by a factor $\sim 10^{10}$. This translates to a magnetic field of the order of $B_{\rm NS} \sim \unit[10^{12}]{G}$ for a newborn neutron star, in line with current estimates.
A second hypothesis is that a strong magnetic field originates dynamically from a dynamo process. During the formation of the proto-neutron star, the magnetic field could be amplified by electric currents generated from rapid rotation or turbulent convective motions of conductive material inside the proto-neutron star a few seconds after its formation \citep[see e.g.][]{Burrows1987, Burrows1988, Duncan1992, White2022}. Probably both effects play a role in the creation of such intense magnetic fields.
% See: https://ui.adsabs.harvard.edu/abs/2008A%26A...479..167N/abstract

%--------------------------------------------------------------------------------------------

\section{The neutron star zoo} \label{sec:ch1_ns_zoo}

%----------------------------------------------------
\begin{figure}
\centering
\includegraphics[width =\textwidth]{P-Pdot_diagram.pdf}
\caption[$P - \dot{P}$ diagram]{$P - \dot{P}$ diagram showing the spin period derivative {\it vs} spin period for the detected neutron stars \citep[Data from the ATNF Pulsar Catalog, \url{https://www.atnf.csiro.au/research/pulsar/psrcat/};][]{Manchester2005}.}
\label{fig:ch1_PPdot_diagram} 
\end{figure}  
%----------------------------------------------------

Figure~\ref{fig:ch1_PPdot_diagram} shows the observed population of non-accreting neutron stars in the $P-\dot{P}$ plane (where $P$ is the neutron star spin period and $\dot{P}$ is the spin period derivative with respect to time). Assuming a dipolar spin-down mechanism we also overlay the lines of constant polar magnetic field at the surface (\textit{solid lines}) (see Equation~\eqref{eq:ch2_Bpol_vacuum}) and characteristic age (\textit{dashed lines}) (see Equation~\eqref{eq:ch2_characteristic_age_approx}) as a reference.
Around $\sim 3000$ neutron stars are known to date and according to their observational properties we classify them as different types. This section will provide an overview of the different classes of neutron stars and their distinguishing characteristics \citep[see][for a more exhaustive review]{Kaspi2010, Harding2013}.

\subsection{Rotation-powered pulsars}

The bulk of the population is composed of \acf{RPPs} (\textit{red dots}). As they spin down due to magnetospheric torques, the loss of rotational energy is converted into particle acceleration which in turn produces broadband electromagnetic emission, from radio to X-rays and gamma-rays. 
The origins of the radio and gamma-ray emission of pulsars are however not well understood. The radio emission is thought to be generated close to the neutron star surface in a narrow beam centred on the magnetic axis within the magnetic pole region of the pulsar (see Section~\ref{sec:ch2_radio_em_geometry}).
The high-energy gamma-ray emission is instead thought to be generated in the outer regions of the neutron star magnetosphere close to the light cylinder where the magnetic field lines open up (see also Section~\ref{sec:ch2_magnetosphere}).
Since the discovery of the first neutron star through its radio pulsations \citep{Hewish1968} around $\sim 2000$ radio pulsars have been detected. 
For some of them, X-ray, gamma-ray and optical pulsations were soon discovered by folding the time series obtained at these wavelengths at the spin periods found in the radio band. At present, there are over 100 \acs{RPPs} detected at X-ray energies and over 300 gamma-ray pulsars \citep{Abdo2013, Smith2023}. While most were found using the ephemerides of already known radio pulsars, many were discovered through their X-ray or gamma-ray pulsations and are radio-quiet. \\
Young neutron stars populate the top part of the diagram. They are often associated with Supernova Remnants (SNRs) (\textit{black stars}) and are often also detected as high-energy gamma-ray pulsars (\textit{purple squares}). As they spin down and their magnetic fields decay in time (see Section~\ref{sec:ch2_B_evol}, pulsars move towards the bottom right region of the diagram.
There are two main populations of RPPs. "Normal" pulsars with spin periods $P \gtrsim \unit[0.1]{s}$ and characteristic ages $\tau \lesssim \unit[100]{Myr}$, occupy the central part of the diagram whereas millisecond pulsars (MSPs), with spin periods down to a few milliseconds and generally higher characteristic ages $\tau \gtrsim \unit[100]{Myr}$ stretch towards the bottom left part of the diagram. MSPs are believed to be older neutron stars mostly in binary system, originally members of the normal RPP population, spun down for tens of Myr and then recycled, i.e., spun up by accretion from their binary companion \citep{Bhattacharya1991, Tauris1999, Tauris2012}.
There is another subpopulation of \acs{RPPs} known as \acf{RRATs} (\textit{light blue triangles}). They were discovered as powerful short-lasting radio bursts that seemed to recur randomly over timescales of minutes to hours \citep{McLaughlin2006}. By studying the arrival times of these bursts common periodicities have been discovered hinting to the spin periods of the emitting neutron stars. \acs{RRATs} have been interpreted as normal pulsars showing an irregular, sporadic emission of radio pulses (detected as radio bursts), instead of a regular emission associated with the rotation period. For these characteristics they are difficult to detect but they should be common in the neutron star population.

\subsection{Magnetars}

Neutron star emission can also be powered by magnetic energy. This is the case for the so-called magnetars, historically also known as \acf{SGRs} and \acf{AXPs} \citep{Woods2006}, which populate the upper-right corner of the $P-\dot{P}$ diagram (\textit{green triangles}). Magnetars have incredibly strong magnetic fields estimated to exceed $\unit[10^{14}]{G}$. This immense magnetic energy reservoirs often result in sporadic bursts of X-rays and gamma-rays which are thought to be caused by the magnetic field decay and significant magnetic field readjustments in the star's crust, leading to starquakes and intense releases of energy \citep[see][for reviews]{Kaspi2017, Esposito2021}.

\subsection{Thermally emitting neutron stars}

Some neutron stars emit thermal radiation, primarily in the form of X-rays, due to their high surface temperatures. These objects are collectively referred to as thermally emitting neutron stars (\textit{yellow triangles}). They include two main subclasses: \acf{CCOs} and the \acf{XDINSs}. \acs{CCOs} are found near the centres of supernova remnants and therefore should be young neutron stars with ages not exceeding a few tens of kyrs. However, they have low $\dot{P}$ values which translate into a low inferred magnetic fields in the dipole braking scenario. A possible explanation for this could be that their fields have been buried during an episode of fallback accretion of debris after the supernova explosion \citep{Shabaltas2012, Vigano2012b, TorresForne2016}. \acs{XDINSs} are also called the magnificent seven and are among the closest neutron stars that we know (few hundred parsecs from the Earth) \citep[see][for reviews]{vanKerkwijk2007, Turolla2009}. Only six of them have measured timing properties. Their thermal emission comes directly from the neutron star surface and is mainly powered by the residual heat stored in their interior and by Ohmic dissipation of the magnetic field in the neutron star crust. Therefore the study of thermally emitting neutron stars provides valuable insights into the cooling mechanisms and interior composition of neutron stars \textbf{REF?}.

\vspace{5mm}

The strict distinction between these different neutron star classes has started to be questioned after some recent discoveries.
For example, the dichotomy between rotational-powered pulsars and magnetars has been softened because magnetar-like X-ray activity was found in pulsars with large rotational energy loss rates, such as PSR J1846--0258 \citep{Gavriil2008} and PSR J1119--6127 \citep{Archibald2016}. Moreover pulsed radio emission has now been detected from several magnetars in outburst like XTE J1810--197 \citep{Camilo2006},  AXP J1810--197 \citep{Kramer2007} and J1818.0--1607 \citep{Esposito2020}. 

Furthermore recent radio surveys, in particular thanks to new radio interferometers such as the LOw Frequency ARray \citep[LOFAR;][]{VanHaarlem2013}, MeerKAT \citep{Jonas2009}, The Australian SKA Pathfinder \citep[ASKAP;][]{Hotan2021}, and the Murchison Widefield Array \citep[MWA;][]{Tingay2013, Wayth2018}, have started to uncover the existence of a new population of mysterious radio sources with very long period that challenge our understanding of the pulsar population and its evolution.
A $\sim\unit[76]{s}$ radio pulsar \citep[\mtp,][]{Caleb2022} and two peculiar coherent radio transients with a periodicity of $\sim\unit[1091]{s}$ \citep[\gleamfirst;][]{Hurley-Walker2022a} and $\sim \unit[1318]{s}$ \citep[\gpm][]{Hurley-Walker2023} have been discovered. The nature of these two latter sources is still debated.
Furthermore, a few years ago the X-ray emitting neutron star \rcw\ at the centre of the $\unit[2]{kyr}$-old supernova remnant RCW103, with a measured modulation of $\sim \unit[6.67]{hr}$, showed a large magnetar-like X-ray outburst \citep{Rea2016, D'Ai2016b}, demonstrating the source's isolated magnetar nature despite its long period and young age. 
We will explore possible scenarios to produce long period pulsars, by considering spin-down induced on a neutron star by the interaction with supernova fallback matter (see Chapter~\ref{Chapter4}) and performing population synthesis studies of neutron stars and magnetic white dwarfs (see Chapter~\ref{Chapter5}).
These discoveries overall are showing that the boundaries between the different neutron star classes are blurring and motivate theoretical frameworks that consider the different neutron star types in an evolutionary scenario. 


%----------------------------------------------------

\section{The birth rate and the need for an evolutionary scenario}

As neutron stars are born from the core collapse of massive OB stars, their birth rate should not exceed the \acf{CCSN} rate in the Milky Way.
The Galactic \acs{CCSN} rate can be estimated via different methods:
\begin{itemize}
    \item \cite{Reed2005} performed a census of the massive stars (with mass $M \gtrsim 10$ \msun) in the solar neighbourhood. From this sample, they extrapolated a Galactic \acs{CCSN} rate between 1 and 2 supernovae per century.
    \item \cite{Li2011} studied the \acs{CCSN}e in the local Universe and by assuming that the Milky Way has similar properties as other galaxies with the same morphological type they derived a \acs{CCSN} rate of $2.30 \pm 0.48$ per century.
    \item \cite{Diehl2006} modelled the gamma-ray emission from radioactive $^{26}$Al in the Milky Way by assuming that this emission traces the ongoing nucleosynthesis pollution by \acs{CCSN}e in the Milky Way. They estimated in this way a \acs{CCSN} rate of $1.9 \pm 1.1$ per century in our Galaxy. 
\end{itemize}

By combining these different ways of estimating the Galactic \acs{CCSN} rate, a recent study from \cite{Rozwadowska2021} found a best estimate of $\mathcal{R}_{\rm CCSN} = 1.79 \pm 0.55$ per century. The birth rate of Galactic neutron star should therefore be compatible with this estimate and not exceed this value.

In the past, several works have used the population of radio pulsars to make estimates of their birth rate.
Historically, pulsar population analyses used the fact that the typical timescales on which neutron stars are active as radio pulsars are much shorter than the age of the Galaxy. In this way, the population can be considered in a steady state and can be viewed as "flowing" in the $P-\dot{P}$ diagram as a "current" obeying a continuity equation \citep{Phinney1981, Vivekanand1981}. At a given spin period $P'$, this current, $J(P')$, equals the pulsar birth rate, $\mathcal{R}_{\rm birth}$, minus the pulsar death rate, $\mathcal{R}_{\rm death}$, in the period range from zero to the actual spin period $P'$, i.e.: 
%------------------------------------------------------------------------
\begin{align}
    J(P') = \mathcal{R}_{\rm birth}(0 < P < P') - \mathcal{R}_{\rm death}(0 < P < P').
\end{align}
%------------------------------------------------------------------------
As the known radio pulsar population is flux-limited (depending on the discovery survey), the maximum value of $J(P)$ provides a lower limit on the pulsar birth rate. For example, \cite{Lorimer2006}, using 1008 non-recycled pulsars detected by the Parkes Low-Latitude Survey estimated a birth rate of $1.38 \pm 0.21$ per century with this method. The advantage of this approach to compute birth rates is that it is agnostic to the details of how pulsars evolve in time.

A second approach to estimate pulsar birth rates is using population synthesis, discussed in detail below. Contrary to the previous approach, population synthesis relies on assuming physical models to describe pulsar properties and how the pulsar population evolves in time. 
For example, \cite{Faucher2006} use Monte Carlo simulations to model the birth properties of pulsars (velocity distributions, spin periods, magnetic fields) and the detectability in the Parkes and Parkes Swinburne Multibeam radio pulsar surveys. They evolve the initial population in time to obtain an observed synthetic pulsar sample to compare with observational data. In this way, they obtain a higher pulsar birth rate of $2.8 \pm 0.5$ per century compared to \cite{Lorimer2006}. 

We note that even without considering the existence of other neutron star classes, we are already at the limit of being compatible with the \acs{CCSN} rate. \cite{Keane2008} highlight that if one takes into account the birth rates estimated for other classes of neutron stars like \acs{RRATs}, \acs{XDINSs} and magnetars (see Section~\ref{sec:ch1_ns_zoo}), the total neutron star birth rate would exceed the Galactic \acs{CCSN} rate by a factor of $\sim 5 - 10$. Furthermore, the recent discovery of very long-period radio sources (see Chapters~\ref{Chapter4} and~\ref{Chapter5}) will further increase this discrepancy if their origin is associated with neutron stars. 
A possible solution is to consider an evolutionary scenario that introduce relationships between the different neutron star classes. Indeed by taking into account the coupled evolution of the magnetic field and the temperature in neutron stars, \cite{Vigano2013} explain the emission from magnetars, XDINs, CCOs and the X-ray emitting rotational powered pulsars as manifestations of neutron stars of different ages and with different magnetic-field strengths and geometries.

%----------------------------------------------------

\section{Population Synthesis: current state of the art}
\label{sec:ch1_popsyn}

Population synthesis models aim to reproduce the observed population of neutron stars by simulating their formation, evolution, and observable properties. 
Typically the adopted approach relies on Monte Carlo simulations to model the different properties of neutron stars from some parametric distributions. These properties are then evolved in time through analytical and numerical models. Finally, models for the observational biases and filters are applied to assess which neutron stars can be detected to build a synthetic observed population.
The simulation outcomes are then compared to the empirical observed data to assess the validity of theoretical models, constrain model parameters and gain insights into the underlying physics.

Due to the abundance of data in the radio band, many works on population synthesis have mainly focused on reproducing the radio pulsar population, in particular trying to constrain the birth spin period and magnetic field distributions.
Some notable research papers in this area include \cite{Narayan1990, Faucher2006, Gonthier2007, Kiel2008, Kiel2009, Oslowski2011, Levin2013, Gullon2014, Bates2014, Cieslar2020}.
Various techniques have been employed to perform parameter optimisation. For example, \cite{Gonthier2007} tried to optimize relevant input physics by hand, tweaking the simulation parameters to obtain a good comparison with observations "by eye". \cite{Narayan1990} and \cite{Faucher2006} used the $\chi^2$ metric and Kolmogorov-Smirnov (KS) tests to compare the simulated distributions with the observed ones. These methods manifest some limitations as the computation of $\chi^2$-statistics rely on having a good amount of data while the KS-test is not particularly sensitive when applied to multi-dimensional distributions of data.
In recent years, improved modelling of neutron star magnetic field evolution and decay, refined cooling models, increased amounts of empirical data and the development of Bayesian techniques like Markov Chain Monte Carlo (MCMC) have all contributed to refining population synthesis codes. Current research efforts aim to combine the information coming from multi-wavelength observations, to better constrain the properties of the neutron star population as a whole and refine theoretical models.
A first attempt to include a more realistic magnetic field evolution based on magneto-thermal simulations of neutron stars and to consider both the radio and the X-ray pulsar population in a population synthesis study was performed by \cite{Gullon2014, Gullon2015} by using annealing methods for optimisation.
However, degeneracies between the simulation parameters were found and it was difficult to put meaningful constraints on the birth rate, especially for magnetars. \cite{Johnston2020} performed a population synthesis study combining both radio and gamma-ray pulsars and showed that highly energetic gamma-ray pulsars and young radio pulsars might come from the same underlying population. 
\cite{Cieslar2020} reproduce the observed radio pulsar population using MCMC, although using a simulation framework with simplified physical models.

This thesis work represents the first efforts to developing a population synthesis approach for isolated neutron stars in conjunction with modern deep-learning techniques. Indeed deep learning can be a powerful tool for extracting relevant features from data coming from different surveys and performing parameter inference (Chapter~\ref{Chapter3}). In this work, we will focus on the radio pulsar population to benchmark our population synthesis approach and compare the results with previous ones in the literature. In particular, we will focus on predicting the birth properties, i.e., spatial and kick-velocity distributions (Chapter~\ref{Chapter6}) and initial spin period and magnetic field distributions and magnetic field evolution (Chapter~\ref{Chapter7}). In Chapter~\ref{Chapter4} and~\ref{Chapter5} we will investigate the nature of recently discovered long-period radio sources assuming a neutron-star or white-dwarf origin scenarios. 

In the following, we describe the theoretical models behind the current understanding of the physical properties of neutron stars, that are fundamental to simulating the radio pulsar population.

%--------------------------------------------------------------------------------------------





